Breadth-first serialisation of trees and rational languages

We present here the notion of breadth-first signature and its relationship with numeration system theory. It is the serialisation into an infinite word of an ordered infinite tree of finite degree. We study which class of languages corresponds to which class of words and,more specifically, using a known construction from numeration system theory, we prove that the signature of rational languages are substitutive sequences.

==> js_beamer4.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                           %
%                   js_beamer.tex                           %
%                                                           %
%       Fichier general de macros  ˆ utiliser avec          %
%                   la classe beamer                        %
%                                                           %
%                    040530                                 %
%                                                           %
%                                                           %
%  041203 call \jscolor flag  (for obvious purpose)         %
%                                                           %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\PointTiret}{\quad}
\newcommand{\jscitation}[1]{\ifthenelse{\equal{#1}{}}% \, 
   {}{{\upshape[\textbf{#1}]\hspace*{0.5em}}}}
%
\newcommand{\NomTheorem}{Thm.}
\newcommand{\NomProposition}{Proposition}
\newcommand{\NomRemark}{Remark}
\newcommand{\NomDefinition}{Def.}
\newcommand{\NomFact}{Fact}
\newcommand{\NomProblem}{Problem}
\newcommand{\NomQuestion}{Question}
%
\newtheorem{remark}{\NomRemark}
\newtheorem{proposition}{{\NomProposition}}
\newtheorem{question}{{\NomQuestion}}
\newtheorem{conjecture}{Conjecture}
\newtheorem{observation}{Observation}
% \newtheorem{problem}{{\NomProblem}}
% \newtheorem{fact}{{\NomFact}}
% \newtheorem{definition}{\NomDefinition}
\newcommand{\DE}[2]{%
   \begin{definition}\label{d.#1}{\jscitation{#2}}\PointTiret\ignorespaces}
\newcommand{\DEF}{\end{definition}}
\newcommand{\PR}[2]{\begin{proposition}\label{p.#1}%  
   {\jscitation{#2}}\PointTiret\ignorespaces}
\newcommand{\PRF}{\end{proposition}}
\newcommand{\LE}[2]{\begin{lemma}\label{l.#1}%  
   {\jscitation{#2}}\PointTiret\ignorespaces}
\newcommand{\LEF}{\end{lemma}}
\newcommand{\COR}[2]{\begin{corollary}\label{c.#1}%  
   {\jscitation{#2}}\PointTiret\ignorespaces}
\newcommand{\CORF}{\end{corollary}}
\newcommand{\RE}[1]{\begin{remark}\label{r.#1}%  
   \PointTiret\ignorespaces}
\newcommand{\REF}{\end{remark}}
\renewcommand{\TH}[2]{\begin{theorem}\label{t.#1}% \TH est deja pris dans Latex 2e  
   {\jscitation{#2}}\PointTiret\ignorespaces}
\newcommand{\THF}{\end{theorem}}
%
\newcommand{\FAC}[2]{\begin{fact}\label{fc.#1}%
   {\jscitation{#2}}\PointTiret\ignorespaces}
\newcommand{\FACF}{\end{fact}}
%
\newcommand{\PRO}[2]{\begin{problem}\label{pb.#1}%  
   {\jscitation{#2}}\PointTiret\ignorespaces}
\newcommand{\PROF}{\end{problem}}
%
\newcommand{\QUE}[2]{\begin{question}\label{pb.#1}%  
   {\jscitation{#2}}\PointTiret\ignorespaces}
\newcommand{\QUEF}{\end{question}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% \section{macros de mep}
%  Macros pour la mise en page
%  espaces de lignes negatifs
\newcommand{\bigskipneg}{\vspace*{-5ex}} %960728
\newcommand{\medskipneg}{\vspace*{-2ex}} %960728
\newcommand{\smallskipneg}{\vspace*{-1ex}} %960728
\newcommand{\miniskipneg}{\vspace*{-0.25ex}} %960728
\newcommand{\equskipneg}{\vspace*{-4ex}} %960728
%%%%%% \section{mac. listes}
\newcommand{\jsListe}[1]%
    {\noindent\makebox[\parindent][r]{{\rm (#1)}}\hspace*{.8em}\ignorespaces}
\newcommand{\thi}{\jsListe{i}}
\newcommand{\thii}{\jsListe{ii}}
\newcommand{\thiii}{\jsListe{iii}}
\newcommand{\thiv}{\jsListe{iv}}
\newcommand{\thv}{\jsListe{v}}
\newcommand{\thvi}{\jsListe{vi}}
\newcommand{\thip}{\jsListe{i'}}
\newcommand{\thiip}{\jsListe{ii'}}
\newcommand{\thiiip}{\jsListe{iii'}}
\newcommand{\thivp}{\jsListe{iv'}}
\newcommand{\thvp}{\jsListe{v'}}
\newcommand{\thvip}{\jsListe{vi'}}
\newcommand{\pointn}{\noindent \makebox[1.2em]{$\bullet$}\ignorespaces}
\newcommand{\pointdn}{\makebox[2.4em]{$\bullet$}}
%
\newcommand{\tha}{\jsListe{a}}
\newcommand{\thb}{\jsListe{b}}
\newcommand{\thc}{\jsListe{c}}
\newcommand{\thd}{\jsListe{d}}
\newcommand{\thejs}{\jsListe{e}}
\newcommand{\thf}{\jsListe{f}}
\newcommand{\thg}{\jsListe{g}}
%%%%
\newlength{\HiddenWordWidth}
\newcommand{\NoDim}[2][l]{\makebox[0pt][#1]{\smash{#2}}}
\newcommand{\NoDimMath}[2][c]{\makebox[0pt][#1]{\smash{\SldMath{#2}}}}
\newcommand{\HiddenDimMath}[2][c]{\makebox[\HiddenWordWidth][#1]{$#2$}}
\newcommand{\FixedDimBox}[3][l]%
   {\settowidth{\HiddenWordWidth}{#2}%
    \makebox[\HiddenWordWidth][#1]{#3}}
\newcommand{\FixedDimBoxl}[2]{\FixedDimBox[l]{#1}{#2}}%
\newcommand{\FixedDimBoxc}[2]{\FixedDimBox[c]{#1}{#2}}%
\newcommand{\FixedDimBoxr}[2]{\FixedDimBox[r]{#1}{#2}}%
\newcommand{\HiddenDimBox}[2][l]{\makebox[\HiddenWordWidth][#1]{#2}}
% 
\newcommand{\PushLine}{~\hfill~}
% \newcommand{\PushLine}{\hbox{}\hfill\hbox{}}
%
\newcommand{\BmrWait}{\addtocounter{beamerpauses}{1}}
\newcommand{\BmrPass}{\addtocounter{beamerpauses}{-1}}
%
\ifjscolor % 
\newcommand{\mathcolor}{green!40!black}
\newcommand{\ImplColor}{\color{RedOrange}}
\newcommand{\EmphColor}{\color{blue}}
\else
\newcommand{\mathcolor}{black}
\newcommand{\ImplColor}{\color{black}}
\newcommand{\EmphColor}{\color{black}}
\fi 
%
\newcommand{\MathColor}{\color{\mathcolor}}
% 
\newcommand{\SldMath}[1]{{\MathColor $#1$}}
\newcommand{\SldMathSp}[1]{{\MathColor $\msp #1 \msp$}}
\newcommand{\SldMathinMath}[1]{{\MathColor #1}}
\newenvironment<>{SldMathEnv}{\MathColor%
                              \smallskipneg
%                               \smallskipneg%
			      }{%
% 			      \smallskipneg
			      \smallskipneg%
			      }
\newenvironment<>{SldEQ}{\MathColor%
%                          \medskipneg%
			 \begin{equation*}}%
			{\end{equation*}}
% 			 
% 			 \medskipneg}
\newcommand{\SldIff}%
    {{\ImplColor{$\e \pmb{\Longleftrightarrow} \e $}}}
\newcommand{\SldImpl}%
    {{\ImplColor{$\e \pmb{\Longrightarrow} \e $}}}

\newcommand{\emphSld}[1]{{\EmphColor \emph{#1}}}
%
\renewcommand{\CompAuto}[1]%
    {%
     \settodepth{\vbd}{\mbox{$\displaystyle{#1\strut}$}}%
     \settoheight{\vbh}{\mbox{$\displaystyle{#1\strut}$}}%
     \setlength{\vbt}{\vbh}\addtolength{\vbt}{\vbd}%
     {}%
     \psline[linewidth=0.8pt,linecolor=\mathcolor]{c-c}(0,-.65\vbd)(0,.9\vbh)%
     \kern1pt%    
     {#1}%
     \kern1pt%
     \psline[linewidth=0.8pt,linecolor=\mathcolor]{c-c}(0,-.65\vbd)(0,.9\vbh)%
     \kern0.4pt%
     }%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput

==> js_environments3.tex <==
% -*- coding: mac-roman -*-
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%                 js_environments3.tex
%
%   Nouvelle formule : part 2 aprs la dŽfinition des environnements
%
% 091109  reconstruction of a file independant from ETA
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%\section{cross-referencing} %%%%%%%%%%%%%%%%%%%
% r\'ef\'erences crois\'ees (entre chapitres diff\'erents)
% 990516 c\'esure pour hyp\'enation
%%%%%%% references to an item  following mnemonic code is used:
%%% 1)  First five letters of the (French) name of the item is used:
%%%        eg  corol  for  corollaire,  exemp  for exemple
%%% 2)  five letters in lower case gives full name,
%%%        capitalised in English only
%%% 3)  first letter in upper case gives abbreviated name,
%%%        capitalised in both English and French
%%% 4)  first letter in upper case, and the five followed by P
%%%        gives abbreviated name (capitalised), followed by the page
%%%        reference
%%% 5)  first TWO letters in upper case, gives full name,
%%%        capitalised in both English and French
%%%
%%%   references listed in alphabetical order
%%%   references have 2 parameters:
%%%     the first one is the chapter ref and is implicitely void,
%%%     for reference call in the same chapter
%%%     the second one is the reference name which is prefixed
%%%     according to the kind of item referenced, which allows to
%%%     give the same name to items of different king and still get
%%%     no confusion.
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%  mod. 060813  addition reference to items inside a remark, an 
%%%  example, etc.
\ifenglish
\newcommand{\dex}[1]{\xmd(#1)}
\fi
\iffrench
\newcommand{\dex}[1]{~#1}
\fi
%%%%%%%\subsection{english cross-ref} %%%%%%%%%%%%%%%%%%%
\ifenglish
% 060809 tuning space
\newcommand{\PageRef}[1]{p.\xmd\pageref{#1}}%020422
\newcommand{\PpageRef}[1]{pp.\xmd\pageref{#1}}%040907
\newcommand{\PPageRef}[2]{pp.\xmd\pageref{#1}--\pageref{#2}}%021212
%
\newcommand{\corol}[2][{}]{Corollary~{#1}\ref{c.#2}}%
\newcommand{\COrol}[2][{}]{Corollary~{#1}\ref{c.#2}}%
\newcommand{\Corol}[2][{}]{Cor.~{#1}\ref{c.#2}}
\newcommand{\CorolP}[2][{}]{Cor.~{#1}\ref{c.#2}, \PageRef{c.#2}}
%
\newcommand{\defin}[2][{}]{Definition~{#1}\ref{d.#2}}%
\newcommand{\DEfin}[2][{}]{Definition~{#1}\ref{d.#2}}%
\newcommand{\Defin}[2][{}]{Def.~{#1}\ref{d.#2}}%
\newcommand{\DefinP}[2][{}]{Def.~{#1}\ref{d.#2}, \PageRef{d.#2}}%
%
\newcommand{\equat}[2][{}]{Equation~({#1}\ref{q.#2})}%
\newcommand{\EQuat}[2][{}]{Equation~({#1}\ref{q.#2})}%
\newcommand{\Equat}[2][{}]{Equat.~({#1}\ref{q.#2})}
\newcommand{\EquatP}[2][{}]{Equat.~({#1}\ref{q.#2}), \PageRef{q.#2}}
\newcommand{\equnm}[2][{}]{({#1}\ref{q.#2})\xspace }
\newcommand{\EqunmP}[2][{}]{({#1}\ref{q.#2}), \PageRef{q.#2}}
%%% 060814  for a typo correction in I.6.2.2
\newcommand{\equnmnosp}[2][{}]{({#1}\ref{q.#2})}
%
\newcommand{\exemp}[2][{}]{Example~{#1}\ref{e.#2}}%
\newcommand{\EXemp}[2][{}]{Example~{#1}\ref{e.#2}}%
\newcommand{\Exemp}[2][{}]{Exam.~{#1}\ref{e.#2}}%
\newcommand{\ExempP}[2][{}]{Exam.~{#1}\ref{e.#2}, \PageRef{e.#2}}%
%
\newcommand{\exerc}[2][{}]{Exercise~{#1}\ref{x.#2}}%
\newcommand{\EXerc}[2][{}]{Exercise~{#1}\ref{x.#2}}%
\newcommand{\Exerc}[2][{}]{Exer.~{#1}\ref{x.#2}}
\newcommand{\ExercP}[2][{}]{Exer.~{#1}\ref{x.#2}, \PageRef{x.#2}}
%
\newcommand{\faitxx}[2][{}]{Fact~{#1}\ref{fc.#2}}%??? do not follow
\newcommand{\Fait}[2][{}]{Fact~{#1}\ref{fc.#2}}%
\newcommand{\FaitP}[2][{}]{Fact~{#1}\ref{fc.#2}, \PageRef{fc.#2}}%
%
\newcommand{\figur}[2][{}]{Figure~{#1}\ref{f.#2}}%
\newcommand{\FIgur}[2][{}]{Figure~{#1}\ref{f.#2}}%
\newcommand{\Figur}[2][{}]{Fig.~{#1}\ref{f.#2}}
\newcommand{\FigurP}[2][{}]{Fig.~{#1}\ref{f.#2}, \PageRef{f.#2}}
%
\newcommand{\lemme}[2][{}]{Lemma~{#1}\ref{l.#2}}%
\newcommand{\LEmme}[2][{}]{Lemma~{#1}\ref{l.#2}}%
\newcommand{\Lemme}[2][{}]{Lem.~{#1}\ref{l.#2}}
\newcommand{\LemmeP}[2][{}]{Lem.~{#1}\ref{l.#2}, \PageRef{l.#2}}
%
\newcommand{\nnote}[2][{}]{Note~{#1}\ref{n.#2}}%
\newcommand{\Nnote}[2][{}]{No\-te~{#1}\ref{n.#2}}
\newcommand{\NnoteP}[2][{}]{No\-te~{#1}\ref{n.#2}, \PageRef{n.#2}}
%
\newcommand{\probl}[2][{}]{Problem~{#1}\ref{pb.#2}}%
\newcommand{\Probl}[2][{}]{Prob.~{#1}\ref{x.#2}}%
\newcommand{\ProblP}[2][{}]{Prob.~{#1}\ref{x.#2}, \PageRef{x.#2}}%
%
\newcommand{\propo}[2][{}]{Proposition~{#1}\ref{p.#2}}%
\newcommand{\PRopo}[2][{}]{Proposition~{#1}\ref{p.#2}}%
\newcommand{\Propo}[2][{}]{Prop.~{#1}\ref{p.#2}}
\newcommand{\PropoP}[2][{}]{Prop.~{#1}\ref{p.#2}, \PageRef{p.#2}}
%
\newcommand{\prpri}[2][{}]{Property~{#1}\ref{pp.#2}}%
\newcommand{\PRpri}[2][{}]{Property~{#1}\ref{pp.#2}}%
\newcommand{\Prpri}[2][{}]{Propty~{#1}\ref{pp.#2}}%
\newcommand{\PrpriP}[2][{}]{Propty~{#1}\ref{pp.#2}, \PageRef{pp.#2}}%
\newcommand{\prprs}[2][{}]{Properties~{#1}\ref{pp.#2}}%
%%% 060811 reference to properties with index
\newcommand{\prpridex}[3][{}]{Property~{#1}\ref{pp.#2}\xmd(#3)}%
%
\newcommand{\remar}[2][{}]{Remark~{#1}\ref{r.#2}}%
\newcommand{\Remar}[2][{}]{Rem.~{#1}\ref{r.#2}}
\newcommand{\RemarP}[2][{}]{Rem.~{#1}\ref{r.#2}, \PageRef{r.#2}}
%
\newcommand{\schol}[2][{}]{Scholium~{#1}\ref{sc.#2}}%
\newcommand{\Schol}[2][{}]{Schol.~{#1}\ref{sc.#2}}
%
\newcommand{\theor}[2][{}]{Theorem~{#1}\ref{t.#2}}%
\newcommand{\THeor}[2][{}]{Theorem~{#1}\ref{t.#2}}%
\newcommand{\Theor}[2][{}]{Th.~{#1}\ref{t.#2}}%
\newcommand{\TheorP}[2][{}]{Th.~{#1}\ref{t.#2}, \PageRef{t.#2}}%
%
\newcommand{\jssecti}[2][{}]{Section~{#1}\ref{s.#2}}%
\newcommand{\JSsecti}[2][{}]{Section~{#1}\ref{s.#2}}%
\newcommand{\jsSecti}[2][{}]{Sec.~{#1}\ref{s.#2}}
\newcommand{\jsSectiP}[2][{}]{Sec.~{#1}\ref{s.#2}, \PageRef{s.#2}}
%
\newcommand{\jssubsecti}[2][{}]{Subsection~{#1}\ref{s.#2}}%
%%% \jschap instead of \chap for the latter is used by french.sty
%%% \chap (and not \chapi) as it came from an old version
\newcommand{\jschap}[1]{Chapter~\ref{chap.#1}}%
\newcommand{\jsCHap}[1]{Chapter~\ref{chap.#1}}%
\newcommand{\jsChap}[1]{Chap.~\ref{chap.#1}}
%
\fi
%%%%%%%\subsection{french cross-ref} %%%%%%%%%%%%%%%%%%%
\iffrench
%
\newcommand{\PageRef}[1]{p.\xmd \xmd \pageref{#1}}%020422
\newcommand{\PpageRef}[1]{pp.\xmd \xmd \pageref{#1}}%040907
\newcommand{\PPageRef}[2]{pp.\xmd\xmd\pageref{#1}--\pageref{#2}}%021212
%
\newcommand{\corol}[2][{}]{corollaire~{#1}\ref{c.#2}}%
\newcommand{\COrol}[2][{}]{Corollaire~{#1}\ref{c.#2}}%
\newcommand{\Corol}[2][{}]{Cor.~{#1}\ref{c.#2}}
\newcommand{\CorolP}[2][{}]{Cor.~{#1}\ref{c.#2}, \PageRef{c.#2}}
%
\newcommand{\defin}[2][{}]{d\'e\-fi\-ni\-tion~{#1}\ref{d.#2}}%
\newcommand{\DEfin}[2][{}]{D\'e\-fi\-ni\-tion~{#1}\ref{d.#2}}%
\newcommand{\Defin}[2][{}]{D\'ef.~{#1}\ref{d.#2}}%
\newcommand{\DefinP}[2][{}]{D\'ef.~{#1}\ref{d.#2}, \PageRef{d.#2}}%
%
\newcommand{\equat}[2][{}]{\'e\-qua\-tion~({#1}\ref{q.#2})}%
\newcommand{\EQuat}[2][{}]{\'E\-qua\-tion~({#1}\ref{q.#2})}%
\newcommand{\Equat}[2][{}]{Equat.~({#1}\ref{q.#2})}
\newcommand{\EquatP}[2][{}]{Equat.~({#1}\ref{q.#2}), \PageRef{q.#2}}
\newcommand{\equnm}[2][{}]{({#1}\ref{q.#2})\xspace }
\newcommand{\EqunmP}[2][{}]{({#1}\ref{q.#2}), \PageRef{q.#2}}
%%% 060814  for a typo correction in I.6.2.2
\newcommand{\equnmnosp}[2][{}]{({#1}\ref{q.#2})}
%
\newcommand{\exemp}[2][{}]{exem\-ple~{#1}\ref{e.#2}}%
\newcommand{\EXemp}[2][{}]{Exem\-ple~{#1}\ref{e.#2}}%
\newcommand{\Exemp}[2][{}]{Exem.~{#1}\ref{e.#2}}%
\newcommand{\ExempP}[2][{}]{Exem.~{#1}\ref{e.#2}, \PageRef{e.#2}}%
%
\newcommand{\exerc}[2][{}]{exer\-cice~{#1}\ref{x.#2}}%
\newcommand{\EXerc}[2][{}]{Exer\-cice~{#1}\ref{x.#2}}%
\newcommand{\Exerc}[2][{}]{Exer.~{#1}\ref{x.#2}}
\newcommand{\ExercP}[2][{}]{Exer.~{#1}\ref{x.#2}, \PageRef{x.#2}}
%
\newcommand{\faitxx}[2][{}]{fait~{#1}\ref{fc.#2}}%
\newcommand{\Fait}[2][{}]{Fait~{#1}\ref{fc.#2}}%
\newcommand{\FaitP}[2][{}]{Fait~{#1}\ref{fc.#2}, \PageRef{fc.#2}}%
%
\newcommand{\figur}[2][{}]{fi\-gu\-re~{#1}\ref{f.#2}}%
\newcommand{\FIgur}[2][{}]{Fi\-gu\-re~{#1}\ref{f.#2}}%
\newcommand{\Figur}[2][{}]{Fig.~{#1}\ref{f.#2}}
\newcommand{\FigurP}[2][{}]{Fig.~{#1}\ref{f.#2}, \PageRef{f.#2}}
%
\newcommand{\lemme}[2][{}]{lem\-me~{#1}\ref{l.#2}}%
\newcommand{\LEmme}[2][{}]{Lem\-me~{#1}\ref{l.#2}}%
\newcommand{\Lemme}[2][{}]{Lem.~{#1}\ref{l.#2}}
\newcommand{\LemmeP}[2][{}]{Lem.~{#1}\ref{l.#2}, \PageRef{l.#2}}
%
\newcommand{\nnote}[2][{}]{no\-te~{#1}\ref{n.#2}}%
\newcommand{\Nnote}[2][{}]{No\-te~{#1}\ref{n.#2}}
\newcommand{\NnoteP}[2][{}]{No\-te~{#1}\ref{n.#2}, \PageRef{n.#2}}
%
\newcommand{\probl}[2][{}]{pro\-bl\`eme~{#1}\ref{pb.#2}}%
\newcommand{\Probl}[2][{}]{Prob.~{#1}\ref{x.#2}}%
\newcommand{\ProblP}[2][{}]{Prob.~{#1}\ref{x.#2}, \PageRef{x.#2}}%
%
\newcommand{\propo}[2][{}]{pro\-po\-si\-tion~{#1}\ref{p.#2}}%
\newcommand{\PRopo}[2][{}]{Pro\-po\-si\-tion~{#1}\ref{p.#2}}%
\newcommand{\Propo}[2][{}]{Prop.~{#1}\ref{p.#2}}
\newcommand{\PropoP}[2][{}]{Prop.~{#1}\ref{p.#2}, \PageRef{p.#2}}
%
\newcommand{\prpri}[2][{}]{pro\-pri\'et\'e~{#1}\ref{pp.#2}}%
\newcommand{\PRpri}[2][{}]{Pro\-pri\'et\'e~{#1}\ref{pp.#2}}%
\newcommand{\Prpri}[2][{}]{Propri.~{#1}\ref{pp.#2}}%
\newcommand{\PrpriP}[2][{}]{Propri.~{#1}\ref{pp.#2}, \PageRef{pp.#2}}%
\newcommand{\prprs}[2][{}]{pro\-pri\'et\'es~{#1}\ref{pp.#2}}%
%%% 060811 reference to properties with index
\newcommand{\prpridex}[3][{}]{pro\-pri\'et\'e~{#1}\ref{pp.#2}~#3)}%
%
\newcommand{\remar}[2][{}]{re\-mar\-que~{#1}\ref{r.#2}}%
\newcommand{\Remar}[2][{}]{Rem.~{#1}\ref{r.#2}}
\newcommand{\RemarP}[2][{}]{Rem.~{#1}\ref{r.#2}, \PageRef{r.#2}}
%
\newcommand{\schol}[2][{}]{scho\-lie~{#1}\ref{sc.#2}}%
\newcommand{\Schol}[2][{}]{Schol.~{#1}\ref{sc.#2}}
%
\newcommand{\theor}[2][{}]{th\'eo\-r\`eme~{#1}\ref{t.#2}}%
\newcommand{\THeor}[2][{}]{Th\'eo\-r\`eme~{#1}\ref{t.#2}}%
\newcommand{\Theor}[2][{}]{Th\'eo.~{#1}\ref{t.#2}}%
\newcommand{\TheorP}[2][{}]{Th\'eo.~{#1}\ref{t.#2}, \PageRef{t.#2}}%
%
\newcommand{\jssecti}[2][{}]{sec\-tion~{#1}\ref{s.#2}}%
\newcommand{\JSsecti}[2][{}]{Sec\-tion~{#1}\ref{s.#2}}%
\newcommand{\jsSecti}[2][{}]{Sec.~{#1}\ref{s.#2}}
\newcommand{\jsSectiP}[2][{}]{Sec.~{#1}\ref{s.#2}, \PageRef{s.#2}}
%
\newcommand{\jssubsecti}[2][{}]{sous-sec\-tion~{#1}\ref{s.#2}}%
%%% \jschap instead of \chap for the latter is used by french.sty
%%% \chap (and not \chapi) as it came from an old version
\newcommand{\jschap}[1]{chapitre~\ref{chap.#1}}%
\newcommand{\jsCHap}[1]{Chapitre~\ref{chap.#1}}%
\newcommand{\jsChap}[1]{Chap.~\ref{chap.#1}}
%
\fi
%%%%%%%\subsection{paragraph cross-ref} %%%%%%%%%%%%%%%%%%%
%%% "paragraphe" is more complex for the French and English versions
%%% differ more radically. kept together to witness it more easily
%%%  mod. 040427, 060809 for the space after \S
%%%  mod. 060812  for the command \jsparg
%%%  061116 pas compltement clair. devrait tre plus explicite.
\ifenglish
\newcommand{\jspara}[2][{}]{\S\xmd{#1}\ref{s.#2}}%
\newcommand{\jsparg}[3][{}]{pa\-ra\-graph~{#1}\ref{s.#3}}%
\newcommand{\jsPara}[3][{}]{\S\xmd{#1}\ref{s.#3}} % modifi\'e 040427
\newcommand{\jsParaP}[3][{}]{\S\xmd{#1}\ref{s.#3}, \PageRef{s.#3}} %040427
\fi
\iffrench
\newcommand{\jspara}[2][{}]{pa\-ra\-graphe~{#1}\ref{s.#2}}% 970416
\newcommand{\jsparg}[3][{}]{pa\-ra\-graphe~{#1}\ref{s.#2}~\ref{s.#3}}%
\newcommand{\jsPara}[3][{}]{\S\xmd{#1}\ref{s.#2}~\ref{s.#3}} % 990908
%           % modifi\'e pour faire apparaitre la reference complete
\newcommand{\jsParaP}[3][{}]{\S\xmd{#1}\ref{s.#2}~\ref{s.#3},
                                              \PageRef{s.#3}} %021110
\fi
%%%%%%%%%%%%%%%%%%%%%%%
\endinput
%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> js_formating_macros4.tex <==
% -*- coding: mac-roman -*-
%%%%%%%%%%%%%%%%%% js_formating_macros4 %%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%
%%%%% 120213  adaptation of the corresponding eta macro file
%%%%%         contains
%%%%%             negative vertical space
%%%%%             pushline
%%%%%             mathematical definition of variable height
%%%%%             two column  macros
%%%%%           no  simplified list
%%%%%           no  reduction of matrices
%%%%%         no ifenglish flag
%%%%%         needs ifdraft flag for the two column macros
%%%%%
%%%%% 130811  addition of
%%%%%              marginal notes
%%%%%         needs ifdraft flag for the NoteDraft macro
%%%%%
%%%%% 131202  version 4 
%%%%%         suppression of
%%%%%              marginal notes (c'est dur de contenter tout le 
%%%%%              monde et son pre)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% \section{negative vertical space}
\newcommand{\bigskipneg}{\vspace*{-5ex}} %960728
\newcommand{\medskipneg}{\vspace*{-2ex}} %960728
\newcommand{\smallskipneg}{\vspace*{-1ex}} %960728
\newcommand{\miniskipneg}{\vspace*{-0.25ex}} %960728
\newcommand{\equskipneg}{\vspace*{-4ex}} %960728
%
\newcommand{\miniskip}{\vspace*{0.1ex}} %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\PushLine}{\hbox{}\hfill\hbox{}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% \section{Mathematical definition}%%%
\newlength{\DefiTest}\setlength{\DefiTest}{0pt}%
\newlength{\DefiHeightu}\newlength{\DefiHeightd}%
\newlength{\DefiDepthu}\newlength{\DefiDepthd}%
\newcommand{\Defi}[2]%
    {%
     \settoheight{\DefiHeightu}{${\displaystyle #1}$}%
     \settodepth{\DefiDepthu}{${\displaystyle #1}$}%
     \addtolength{\DefiHeightu}{\DefiDepthu}%
     \settoheight{\DefiHeightd}{${\displaystyle #2}$}%
     \settodepth{\DefiDepthd}{${\displaystyle #2}$}%
     \addtolength{\DefiHeightd}{\DefiDepthd}%
     \left\{#1%
     \rule[-\DefiDepthd]{\DefiTest}{\DefiHeightd}%
     \xmd\right|%
     \left.%
     \rule[-\DefiDepthu]{\DefiTest}{\DefiHeightu}%
      #2\right\}%
     }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% \section{Twocolumns macros}%%% colonne + figure %%%%%%%%
%%% variables
\newlength{\ColoText}% largeur de la colonne "de texte"
\newlength{\ColoFigu}% largeur de la colonne "de figure"
\newlength{\TextFiguSpace}% intervalle entre les deux colonnes
\newlength{\parindenttemp} % for indentation in minipage
\newlength{\parskiptemp} % for alinea spacing in minioage
\newlength{\fboxseptemp} % pour memoriser \fboxsep
\newcommand{\TFBoxing}{}
\newcommand{\TFVertAlig}{}
\newcommand{\LeftLarg}{}
% values
\setlength{\fboxseptemp}{\fboxsep}% parce qu'on va l'annuler en draft
\setlength{\parindenttemp}{\parindent}
\setlength{\parskiptemp}{\parskip}
\setlength{\TextFiguSpace}{1.2em}% intervalle entre les deux colonnes
\renewcommand{\LeftLarg}{.66}
\ifdraft\renewcommand{\TFBoxing}{\fbox}\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% 3 paramtres
%%% 1) largeur de la colonne de gauche, en % de \textwidth
%%%    valeur implicite : \LeftLarg = 2/3
%%% 2) texte de la colonne de gauche
%%% 3) texte de la colonne de droite (souvent une figure)
%%% Boites alignŽes sur le haut,
%%%        encadrŽes en mode draft
\newcommand{\TxtFg}[3]%
   {%
    \setlength{\ColoText}{#1\textwidth}%
    \setlength{\ColoFigu}{\textwidth}%
    \addtolength{\ColoFigu}{-\ColoText}%
    \addtolength{\ColoText}{-.5\TextFiguSpace}%
    \addtolength{\ColoFigu}{-.5\TextFiguSpace}%
    \ifdraft\setlength{\fboxsep}{0pt}\fi% % mod 000912, 050822
%
    \noi
    \TFBoxing{%
       \begin{minipage}[\TFVertAlig]{\ColoText}%
%           \RstBLS% 050822
          \setlength{\parindent}{\parindenttemp}%
          \setlength{\parskip}{\parskiptemp}%
          \par\vspace*{0mm}% pour l'alignement sur le haut
             #2
       \end{minipage}%
             }%
    \hspace*{\TextFiguSpace}%
    \TFBoxing{%
       \begin{minipage}[\TFVertAlig]{\ColoFigu}%
          \par\vspace*{0mm}%
             #3%
       \end{minipage}%
             }%
%
    \ifdraft\setlength{\fboxsep}{\fboxseptemp}\fi%050822
   }%
%%%
\newcommand{\TextFigu}[3][\LeftLarg]%
   {\renewcommand{\TFVertAlig}{t}\TxtFg{#1}{#2}{#3}}
\newcommand{\TextFiguC}[3][\LeftLarg]%
   {\renewcommand{\TFVertAlig}{c}\TxtFg{#1}{#2}{#3}}
%%%%%%%%% Figures vers l'exterieur avec dŽbordement
%%% ie la colonne "de droite" est du cotŽ de la marge
\newcommand{\TextFiguX}[3][\LeftLarg]
   {%
    \setlength{\ColoText}{#1\textwidth}%
    \setlength{\ColoFigu}{\textwidth}%
    \addtolength{\ColoFigu}{-\ColoText}%
    \addtolength{\ColoText}{-.5\TextFiguSpace}%
    \addtolength{\ColoFigu}{-.5\TextFiguSpace}%
    \addtolength{\ColoFigu}{\ETAExtendedLineWidth}% mod 000912,050822
    \ifdraft\setlength{\fboxsep}{0pt}\fi% % mod 000912, 050822
%
    \noi
    \ifodd\value{page}%
       \TFBoxing{%
          \begin{minipage}[t]{\ColoText}%
             \RstBLS% 050822
             \setlength{\parindent}{\parindenttemp}%
             \setlength{\parskip}{\parskiptemp}%
             \par\vspace*{0mm}% pour l'alignement sur le haut
                #2
          \end{minipage}%
                }%
       \hspace*{\TextFiguSpace}%
       \TFBoxing{%
          \begin{minipage}[t]{\ColoFigu}%
             \par\vspace*{0mm}%
                #3%
          \end{minipage}%
                }%
    \else
       \hspace*{-\ETAExtendedLineWidth}% mod 000912
       \TFBoxing{%
          \begin{minipage}[t]{\ColoFigu}%
             \par\vspace*{0mm}%
                #3%
          \end{minipage}%
                }%
       \hspace*{\TextFiguSpace}%
       \TFBoxing{%
          \begin{minipage}[t]{\ColoText}%
             \RstBLS% 050822
             \setlength{\parindent}{\parindenttemp}%
             \setlength{\parskip}{\parskiptemp}%
             \par\vspace*{0mm}% pour l'alignement sur le haut
                #2
          \end{minipage}%
                }%
    \fi%
    \ifdraft\setlength{\fboxsep}{\fboxseptemp}\fi%050822
   }
%%%%%%%%% 2 colonnes egales
%%% Attention! la dŽnomination est trompeuse
%%% car la colonne de droite ne comporte pas de
%%% retrait. Devrait s'appeler "FiguFigu"
\newcommand{\TextText}[2]{\TextFigu[.5]{#1}{#2}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%% \subsection{marginal notes}
% \newcommand{\NoteEnMarge}[1]%
%    {%
%     \marginpar[\begin{flushright}%
%                {\sl {\scriptsize #1}}%
%                \end{flushright}]%
%               {\begin{flushleft}%
%                {\sl {\scriptsize #1}}%
%                \end{flushleft}}%
% 	}%
% %%%
% \newcommand{\NoteDraft}[1]{{\ifdraft\NoteEnMarge{#1}\fi}} %030123-050821
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%% \section{enumeration labels} %%%
% %%% simplified version
% \newlength{\retraita}\setlength{\retraita}{1.5\parindent}
% \newlength{\listespa}\setlength{\listespa}{.8em}
% %
% \newcommand{\EnumLbl}[1]{\rm (#1)}%
% \newcommand{\jsListe}[1]%
%     {\noindent\makebox[\retraita][r]{\EnumLbl{#1}}%
%      \hspace*{\listespa}\ignorespaces}
% %
% \newcommand{\tha}{\jsListe{a}}
% \newcommand{\thb}{\jsListe{b}}
% \newcommand{\thc}{\jsListe{c}}
% \newcommand{\thd}{\jsListe{d}}
% \newcommand{\thejs}{\jsListe{e}}
% \newcommand{\thf}{\jsListe{f}}
% \newcommand{\thg}{\jsListe{g}}
% %
% \newcommand{\thi}{\jsListe{i}}
% \newcommand{\thii}{\jsListe{ii}}
% \newcommand{\thiii}{\jsListe{iii}}
% \newcommand{\thiv}{\jsListe{iv}}
% \newcommand{\thv}{\jsListe{v}}
% \newcommand{\thvi}{\jsListe{vi}}
% %
% \newcommand{\thip}{\jsListe{i$'$}}
% \newcommand{\thiip}{\jsListe{ii$'$}}
% \newcommand{\thiiip}{\jsListe{iii$'$}}
% \newcommand{\thivp}{\jsListe{iv$'$}}
% \newcommand{\thvp}{\jsListe{v$'$}}
% \newcommand{\thvip}{\jsListe{vi$'$}}
% %
% \newcommand{\thnu}{\jsListe{1}}
% \newcommand{\thnd}{\jsListe{2}}
% \newcommand{\thnt}{\jsListe{3}}
% \newcommand{\thnq}{\jsListe{4}}
% %%% to be fixed
% \newcommand{\point}{\makebox[\retraita][l]{$\bullet$}}
% \newcommand{\pointr}{\makebox[\retraita][r]{$\bullet$ \ }}
% \newcommand{\pointn}{\noindent \makebox[1.2em]{$\bullet$}\ignorespaces}
%%% liste d'axiomes
% should be followed with a % for a margin of fixed size
% \jspointtiret defined in eta_environments
\newcommand{\Axio}[1]%
   {\pointn #1\hspace*{.1em}\jspointtiret\hspace*{.4em}\ignorespaces}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%\section{matrices}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Mise en page des grosse matrices
% % valeurs des echelles pour eta
% \newcommand{\redmatu}[1]{\scalebox{0.84}{#1}}
% \newcommand{\redmatd}[1]{\scalebox{0.66}{#1}}
% \newcommand{\redmatt}[1]{\scalebox{0.90}{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> js_macros3.tex <==
% -*- coding: mac-roman -*-
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                           %
%                  js_macros3.tex                           %
%                                                           %
% Remise ˆ plat, et en ordre, du fichier  js_macros3.tex    %
%                                                           %
% Doit permettre la paramŽtrisation des symboles d'alphabet %
%                                                           %
% 070328                                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%% 030120  Mise \`a plat compl\`ete %%%%
% % 030203
% %
% %%%% operateur math %(Paul Gastin) (mod. js 941031; 970919)
% % Grace a \math, on peut, mais il n'est pas necessaire d'utiliser $$.
% % Par exemple, $\N$ et \N donneront (presque) la meme chose.
% % En mode LR, laisse un blanc apres; mathnosp supprime ce blanc
% % mod 991211 utilisation de \xspace pour supprimer l'interet de
% % \mathnosp; de toute facon, je n'utilise plus \math
% \def\math#1{\ifmmode #1\else \mbox{$#1$}\xspace \fi}
% \def\mathnosp#1{\ifmmode #1\else \mbox{$#1$}\fi}
%%%%%%%\section{intervalles}%%%%%%%%%%%%%%%%%%
%  intervalles d'entiers (mod. 971017)
%  mod.9904
%  mod.070328 call to math suppressed
\newcommand{\jsInter}[1]{\mathbf{#1}}
\newcommand{\kinter}{\jsInter{k}}
\newcommand{\linter}{\jsInter{l}}
\newcommand{\hinter}{\jsInter{h}}
%
\newcommand{\jsTerval}[1]{[{#1}]} % 011224 supp. math
\newcommand{\kterval}{\jsTerval{k}}
\newcommand{\hterval}{\jsTerval{h}}
\newcommand{\lterval}{\jsTerval{l}}
\newcommand{\mterval}{\jsTerval{m}}
\newcommand{\nterval}{\jsTerval{n}}
\newcommand{\Nterval}{\jsTerval{N}}
\newcommand{\pterval}{\jsTerval{p}}
\newcommand{\qterval}{\jsTerval{q}}
\newcommand{\rterval}{\jsTerval{r}}
\newcommand{\sterval}{\jsTerval{s}}
%
\newcommand{\jsAvi}[1]{\scalebox{1.2}{\mathfrak{#1}}}
\newcommand{\kAvi}{\jsAvi{k}}
\newcommand{\aAvi}{\jsAvi{a}}
\newcommand{\bAvi}{\jsAvi{b}}
% % entiers sign\'es 021110 c'est le boxon y a deux sortes de
% % lettres barr\'ees cf js_symboles.tex  \abar et \bara
% \newcommand{\jsBar}[1]{{\bar{#1}}}
% \newcommand{\baru}{\jsBar{1}}
% \newcommand{\bard}{\jsBar{2}}
% \newcommand{\bart}{\jsBar{3}}
% \newcommand{\barq}{\jsBar{4}}
% \newcommand{\barl}{\jsBar{l}}
% \newcommand{\barh}{\jsBar{h}}
%
\newcommand{\jsCard}[1]{{\|{#1}\|}}
\newcommand{\fracts}[2]{{\textstyle \frac{#1}{#2}}}
%%%%%%%%%%%%%%%\section{fonctions}%%%%%%%%%%
%  Signes diacritiques constructeurs de fonctions
%   010104
%
%%% extension d'une fonction 030102
\newcommand{\ExtnF}[1]%
   {\overset{{\scriptscriptstyle \pmb{\smile}}}{#1}}
\newcommand{\Extngam}{\ExtnF{\gamma}}
% \newcommand{\jsTop}[1]{\OB{#1}^{\circ}} % pas une bonne id\'ee
\newcommand{\jsTop}[1]{\overset{{\scriptstyle \circ}}{#1}}
\newcommand{\Topa}{\jsTop{\alpha}}
%%% quotient d'une fonction 990728
\newcommand{\jsQuotF}[2]{{#1}{\pmb{/}}\!\raisebox{-.4ex}{$#2$}}
\newcommand{\Qaf}{\jsQuotF{\alpha}{f}}
\newcommand{\Qag}{\jsQuotF{\alpha}{g}}
\newcommand{\Qau}{\jsQuotF{\alpha}{\unAe}}
%%% differentielle d'une fonction 010104
\newcommand{\DiffF}[1]%
   {\overset{{\scriptscriptstyle \pmb{\lor}}}{#1}}
%    {\overset{{\scriptscriptstyle \leftrightharpoons}}{#1}}
\newcommand{\Dal}{\DiffF{\alpha}}
%%% localisation d'une fonction 010118
\newcommand{\LocaF}[1]%
   {\overset{{\scriptscriptstyle \leftrightarrow}}{#1}}
\newcommand{\Lal}{\LocaF{\alpha}}
%
\newcommand{\jsCrocU}[1]{\left[\rule{0pt}{2.8ex} \smash{#1}\right]}
%%%%%%%%%%%%%%%\section{type log}%%%%%%%%%%
%  Fonctions type log (mod. 970917)
%        mise en sans s\'erif 990925 (pour certains)
%        991211  pour d'autres
\newcommand{\Dom}{\mathsf{Dom}\,}
\renewcommand{\Im}{\mathsf{Im}\,}
\newcommand{\Ker}{\mathsf{Ker}\,}
% dimension 000629
\newcommand{\jsDim}[1]{\operatorname{{\mathsf{dim}}_{#1}}}
\newcommand{\Dim}{\jsDim{}}
\newcommand{\DimK}{\jsDim{\K}}
% distance 001023
% \newcommand{\di}{{\rm d}\,}
\newcommand{\jsDist}[2][{}]%
%    {\operatorname{\mathbf{d}_{#1}}(#2)} corr 070313
   {\operatorname{\mathbf{d}_{#1}}\left(#2\right)}
\newcommand{\di}{{\operatorname{\mathbf{d}}}}
\newcommand{\dic}{{\operatorname{\mathbf{c}}}}
\newcommand{\distl}{{\operatorname{\mathbf{l}}}} % 000511
\newcommand{\did}{{\operatorname{\mathsf{d}}}}
%%% distance pr\'efixe 990801
\newcommand{\jsDistP}[1]{\jsDist[p]{#1}}
%%% profondeur d'une expression 010208
\newcommand{\Dept}[1]{\operatorname{\mathsf{d}}(#1)}
% \newcommand{\ec}{{\rm e}\,}
\newcommand{\ec}{{\operatorname{\mathbf{e}}}}
\newcommand{\jsval}{{\operatorname{\mathbf{v}}}}
\newcommand{\Valu}[1]{\jsval (#1)}
% \newcommand{\supp}{{\rm supp}\,}
\newcommand{\supp}{\operatorname{{\mathsf{supp}\,}}}
\newcommand{\Card}{{\rm Card}\,}
\newcommand{\Pre}{{\operatorname{{\mathsf{Pre}}}}}
\newcommand{\Suf}{{\operatorname{{\mathsf{Suf}}}}}
\newcommand{\Fac}{{\operatorname{{\mathsf{Fac}}}}}
\newcommand{\Conj}{{\operatorname{{\mathsf{Conj}}}}}
\newcommand{\jsPer}{\operatorname{{\mathsf{per}}}}% 020528
\newcommand{\Var}{{\rm Var}\,}
\newcommand{\pgcd}{{\operatorname{pgcd}}} % supprime l'arg.
%                                              % 981006
%%% d\'ecalage and such modif 001114
\newcommand{\jsdel}{\operatorname{\mathsf{del}}}
\newcommand{\delp}[1]{\jsdel (#1)}
\newcommand{\jsdec}{\operatorname{\mathsf{lag}}}
\newcommand{\decp}[1]{\jsdec (#1)}
\newcommand{\jsdiv}{\operatorname{\mathsf{lag}}}
\newcommand{\divp}[1]{\jsdiv (#1)}
\newcommand{\jsrang}{\operatorname{\mathsf{r}}}
\newcommand{\Rang}[1]{\jsrang (#1)}
%
\newcommand{\jsRelMat}[1]{{\operatorname{\mathsf{m}}(#1)}}
\newcommand{\arelmat}{\jsRelMat{\alpha}}
%
\newcommand{\jsHaut}[1]{{\operatorname{\mathsf{h}}[#1]}}
\newcommand{\HautGen}[1]{{\operatorname{\mathsf{gsh}}[#1]}}
%
\newcommand{\jsEnla}[1]{{\operatorname{\mathsf{lc}}(#1)}}
%
\newcommand{\iEB}[1]{{\operatorname{\mathsf{i}_{\EBzi}}(#1)}}
\newcommand{\EBC}[1]{{\operatorname{\mathsf{E}_{\BzCi}}(#1)}}
% 000226 reprogrammation de min et max
\renewcommand{\min}{{\operatornamewithlimits{\mathsf{min}}}}
\renewcommand{\max}{{\operatornamewithlimits{\mathsf{max}}}}
\renewcommand{\inf}{{\operatornamewithlimits{\mathsf{inf}}}}
\renewcommand{\sup}{{\operatornamewithlimits{\mathsf{sup}}}}
\renewcommand{\lim}{{\operatornamewithlimits{\mathsf{lim}}}}
\newcommand{\limsp}{{\operatorname{\mathsf{lim}\xmd}}}
%%%%%%%%%%%%%%%%%%%\section{\'equivalences}
\newcommand{\ClasE}[2]{{#1}/{#2}}
% 010105 programmation des classes
\newcommand{\Clas}[2]{[#1]_{#2}}
\newcommand{\Glas}[1]{[{#1}]}% 010213
% 000831 programmation des modulo et des quotients
\newcommand{\mmod}[1]{\e [#1]}
\newcommand{\mmoda}{\mmod{\alpha}}
\newcommand{\qquot}[2]{\ClasE{#1}{#2}}
%%% congruence % 000704 %050826 \Modu supprimŽ
\newcommand{\modu}[1]{\mod #1}
% 010101 ind\'efini
\newcommand{\Inde}{\top}
% 030203 tranches de langages \section{tranche}
\newcommand{\etaFH}[1]{\operatorname{\mathsf{FH}}(#1)}
\newcommand{\etaFT}[1]{\operatorname{\mathsf{FT}}(#1)}
\newcommand{\etaST}[1]{\operatorname{\mathsf{ST}}(#1)}
\newcommand{\FHL}{\etaFH{L}}
\newcommand{\FHg}{\etaFH{g}}
\newcommand{\FTL}{\etaFT{L}}
\newcommand{\STL}{\etaST{L}}
\newcommand{\etaSMl}[1]{{\mathsf{F_{#1}}}}
\newcommand{\etaSM}[2]{\operatorname{\mathsf{F_{#1}}}(#2)}
\newcommand{\FaL}{\etaSM{\alpha}{L}}
%%%%%%%%%%%%%%%%%%%\section{parties de mono\"\i des}
%  Ensembles (semi-anneaux) des parties (mod. 970501)
%
\newcommand{\Pfrak}{\mathfrak{P}}
%
\newcommand{\jsPart}[1]{{\operatorname{\Pfrak}\left(#1\right)}}
\newcommand{\jspart}[1]{\jsPart{#1}} % compatibilit\'e
\newcommand{\jsPartF}[1]{{\Pfrak_{\mathjsu{fin}}(#1)}}
% \newcommand{\jsPartK}[2]{{\Pfrak_{\mathjsu{(#2)}}(#1)}}
\newcommand{\jsPartK}[2]{{\Pfrak_{(#2)}(#1)}}
\newcommand{\jsFin}[1]{#1_{\mathsf{f}}}
\newcommand{\jsInf}[1]{#1_{\infty}}
\newcommand{\tauF}{\jsFin{\tau}}
\newcommand{\tauI}{\jsInf{\tau}}
%
\newcommand{\PdAe}{\jspart{\Ae}}
\newcommand{\PcAe}{\PdAe} % compatibilit\'e
\newcommand{\PdBe}{\jspart{\Be}}
%\newcommand{\PdCe}{\jspart{\Ce}}
\newcommand{\PdE}{\jspart{E}}
\newcommand{\PdF}{\jspart{F}}
\newcommand{\PdM}{\jspart{M}}
\newcommand{\PcM}{\PdM} % compatibilit\'e
\newcommand{\PdN}{\jspart{N}}
\newcommand{\PcN}{\PdN} % compatibilit\'e
\newcommand{\PdQ}{\jspart{Q}}
\newcommand{\PcQ}{\PdQ} % compatibilit\'e
\newcommand{\PdV}{\jsPart{V}}
% Ensemble des applications 990712
% mod 991211 sur les conseils de sylvain
% \newcommand{\Afrak}{\mathfrak{A}}
\newcommand{\jsRela}[1]{{\mathfrak{R}_{#1}}}
\newcommand{\jsGSym}[1]{{\mathfrak{S}_{#1}}}
\newcommand{\jsTran}[1]{{\mathfrak{T}_{#1}}}
% \newcommand{\jsRela}[1]{{\mathfrak{R}(#1)}}
% \newcommand{\jsGSym}[1]{{\mathfrak{S}(#1)}}
\newcommand{\jsTranp}[1]{{\mathfrak{T}(#1)}}
\newcommand{\jsAppl}[1]{{\mathfrak{A}(#1)}}
\newcommand{\FdQ}{\jsTranp{Q}}
\newcommand{\TcS}{\jsTran{S}}
% Ideal (pour un ordre) engendr\'e 001102
% pour remplacer un \WH malheureux
\newcommand{\Idea}[1]{\mathsf{I}(#1)}
%%% complement 981015 (requires amssymb pack.)
\newcommand{\jsComp}[2][{}]{\complement _{#1} #2}
% Def pour le theor EPR 990727
%    compl\'et\'e 991215
\newcommand{\Efrak}{\mathfrak{E}}
\newcommand{\jsEhreN}[2]{{\Efrak_{#2}(#1)}}
\newcommand{\jsEhreNp}[2]{{\Efrak'_{#2}(#1)}}
\newcommand{\jsEhreNk}{{\Efrak_{k}}}
\newcommand{\jsEhreNh}{{\Efrak_{h}}}
\newcommand{\jsEhreNn}{{\Efrak_{n}}}
\newcommand{\jsEhreNpk}{{\Efrak'_{k}}}
\newcommand{\jsEhreNph}{{\Efrak'_{h}}}
\newcommand{\Jfrak}{\mathfrak{J}}
\newcommand{\jsJaff}[2]{{\Jfrak_{#2}(#1)}}
\newcommand{\jsJaffp}[2]{{\Jfrak'_{#2}(#1)}}
\newcommand{\jsJaffk}{{\Jfrak_{k}}}
\newcommand{\jsJaffpk}{{\Jfrak'_{k}}}
\newcommand{\jsJaffh}{{\Jfrak_{h}}}
\newcommand{\jsJaffph}{{\Jfrak'_{h}}}
% \newcommand{\jsEhreN}[2]{{\Efrak_{\mathjsu{#2}}(#1)}}
% Def pour le theor Dejean-Schutz 000104
\newcommand{\Wfrak}{\mathfrak{W}}
\newcommand{\EggSch}[1]{{\Wfrak_{#1}}}
\newcommand{\EggSchk}{\EggSch{k}}
%%% Plus long prefixe commun 990727
\newcommand{\jsPLPC}[2][{}]{\bigwedge _{#1} #2}
\newcommand{\jsPlpc}{\pmb{\land}}
%%%%%%%%%%%%%%%%%\section{semi-anneaux}
% Structure 000702
\newcommand{\StruSA}[1]{\aut{#1}}
%    unit\'es (param\'etr\'ees 000702)
\newcommand{\ETAze}[1]{0_{#1}}
\newcommand{\ETAun}[1]{1_{#1}}
\newcommand{\zeK}{\ETAze{\Kmbb}}
\newcommand{\zeL}{\ETAze{\Lmbb}}
\newcommand{\zeB}{\ETAze{\Bmbb}}
\newcommand{\unK}{\ETAun{\Kmbb}}
\newcommand{\unL}{\ETAun{\Lmbb}}
\newcommand{\unB}{\ETAun{\Bmbb}}
\newcommand{\unT}{\ETAun{\Tmbb}}
\newcommand{\unZ}{\ETAun{\Zmbb}}
%
%%% quotients de \N 010218
\newcommand{\NQuot}[2]{\N_{#1,#2}}
\newcommand{\Nru}{\NQuot{r}{1}}
\newcommand{\Nrp}{\NQuot{r}{p}}
%   Semi-anneaux composes
\newcommand{\x}{\! \times \!}
% exposants
\newcommand{\QpQ}{Q \x Q}
\newcommand{\RpR}{\mathnosp{R \x R}}
%
\newcommand{\BQQ}{{{\B}^{Q \x Q}}}
\newcommand{\BRR}{{{\B}^{R \x R}}}
\newcommand{\BQun}{{{\B}^{Q \x 1}}}
\newcommand{\BQu}{\BQun} % compatibilit\'e
\newcommand{\BunQ}{{{\B}^{1 \x Q}}}
\newcommand{\BuQ}{\BunQ} % compatibilit\'e
%
\newcommand{\KQQ}{{\K}^{Q \x Q}}
\newcommand{\KRR}{{{\K}^{R \x R}}}
\newcommand{\KunQ}{{{\K}^{1 \x Q}}}
\newcommand{\KQun}{{{\K}^{Q \x 1}}}
\newcommand{\KQu}{\KQun} % compatibilit\'e
\newcommand{\KuQ}{\KunQ} % compatibilit\'e
%
\newcommand{\McQQ}{{{\Mc}^{Q \x Q}}}
% centre
\newcommand{\KCent}[1]{{#1}_{\mathsf{c}}}
\newcommand{\Kcent}{\KCent{\K}}
% dual 000703
\newcommand{\Dual}[1]{{#1}^{\star}}
\newcommand{\DDual}[1]{{#1}^{\star \star}}%000908
\newcommand{\Orth}[1]{{#1}^{\pmb{\bot}}}
% groupe des unit\'es 001104
\newcommand{\Uplu}[1]{\mathsf{U}_{+}({#1})}
%%%%%%%%%\section{s\'eries}
% terme constant, partie propre 000911
\newcommand{\TermCnst}[1]{{\operatorname{\mathsf{c}}(#1)}}
\newcommand{\TermCst}[1]{\TermCnst{#1}} %%% compatibility
\newcommand{\PartProp}[1]{#1_{\mathsf{p}}}
\newcommand{\spr}{\PartProp{s}}
%   Semi-anneaux de series  (mod. 970501)
%%% 070328  suppressed
\newcommand{\SerSAnMon}[2]%
    {#1 \langle \! \langle  #2  \rangle \! \rangle }
\newcommand{\SerSAnMonD}[2]%
    {\left[#1\right] \langle \! \langle  #2  \rangle \! \rangle }
\newcommand{\SerMon}[1]%
    {\!\langle \! \langle  #1  \rangle \! \rangle }
\newcommand{\SD}[1]{\SerMon{#1}} % compatibilit\'e
%
\newcommand{\BAe}{\SerSAnMon{\B}{\Ae }}
\newcommand{\BBe}{\SerSAnMon{\B}{\Be }}
\newcommand{\BM}{\SerSAnMon{\B}{M}}
\newcommand{\BN}{\SerSAnMon{\B}{N}}
\newcommand{\BMN}{\SerSAnMon{\B}{M \x N}}
\newcommand{\KAe}{\SerSAnMon{\K}{\Ae }}
\newcommand{\KBe}{\SerSAnMon{\K}{\Be }}
\newcommand{\KCe}{\SerSAnMon{\K}{\Ce }}
\newcommand{\KA}{\KAe} % compatibilit\'e
\newcommand{\KM}{\SerSAnMon{\K}{M}}
\newcommand{\KcM}{\SerSAnMon{\Kcent}{M}}
\newcommand{\KMQQ}{\KM ^{Q \x Q}}
\newcommand{\KN}{\SerSAnMon{\K}{N}}
\newcommand{\KcN}{\SerSAnMon{\Kcent}{N}}
\newcommand{\KMN}{\SerSAnMon{\K}{M \x N}}
\newcommand{\KcMN}{\SerSAnMon{\Kcent}{M \x N}}
\newcommand{\KNeM}{\SerSAnMon{\left[\KN\right]}{M}}
\newcommand{\KMeN}{\SerSAnMon{\left[\KM\right]}{N}}
\newcommand{\KcNeM}{\SerSAnMon{\left[\KcN\right]}{M}}
\newcommand{\KcMeN}{\SerSAnMon{\left[\KcM\right]}{N}}
\newcommand{\KPMexe}{\SerSAnMon{\left[\KPM \right]}{x^{*}}}
\newcommand{\KP}{\SerSAnMon{\K}{P}}
\newcommand{\KcP}{\SerSAnMon{\Kcent}{P}}
\newcommand{\KQQAe}{\SerSAnMon{\KQQ }{\Ae }}
\newcommand{\KQQM}{\SerSAnMon{\KQQ }{M}}
\newcommand{\Kxe}{\SerSAnMon{\K}{x^{*}}}
\newcommand{\LbM}{\SerSAnMon{\Lb}{M}}
\newcommand{\LbMN}{\SerSAnMon{\Lb}{M \x N}}
\newcommand{\Nae}{\SerSAnMon{\N}{a^{*}}}
\newcommand{\NAe}{\SerSAnMon{\N}{\Ae }}
\newcommand{\NBe}{\SerSAnMon{\N}{\Be }}
\newcommand{\NAeBe}{\SerSAnMon{\N}{\Ae \x \Be}}
\newcommand{\NM}{\SerSAnMon{\N}{M}}
\newcommand{\NN}{\SerSAnMon{\N}{N}}
\newcommand{\NMN}{\SerSAnMon{\N}{M \x N}}
\newcommand{\Nxe}{\SerSAnMon{\N}{x^{*}}}
\newcommand{\Naexe}{\SerSAnMon{\N}{a^{*} \x x^{*}}}
\newcommand{\Ncae}{\SerSAnMon{\Nc}{a^{*}}}
\newcommand{\QM}{\SerSAnMon{\Q}{M}}
\newcommand{\QN}{\SerSAnMon{\Q}{N}}
\newcommand{\Qcae}{\SerSAnMon{\Qc}{a^{*}}}
\newcommand{\ZAe}{\SerSAnMon{\Z}{\Ae }}
\newcommand{\ZA}{\ZAe} % compatibilit\'e
%
\newcommand{\McAe}{\SerSAnMon{\Mc}{\Ae}}
%{{{\Mc}\!\! \ll \! \Ae \! \gg}}
\newcommand{\McAte}{\SerSAnMon{\Mc}{\Ate}}
% \newcommand{\McAte}{{{\Mc}\!\! \ll \! \Ate \! \gg}}
% series sur un groupe ordonne
% parametrisation 000319
\newcommand{\etaWO}[1]{{#1}_{\mathsf{wo}}}
\newcommand{\Kwog}{\SerSAnMon{\etaWO{\K}}{G}}
\newcommand{\KwoFA}{\SerSAnMon{\etaWO{\K}}{F(\Alph)}}
\newcommand{\KwoFB}{\SerSAnMon{\etaWO{\K}}{F(\Blph)}}
\newcommand{\KwoFAuk}{\SerSAnMon{\etaWO{\K}}%
                  {F(\Alph_{1})\x \cdots \x F(\Alph_{k})}}
\newcommand{\KwoFAdk}{\SerSAnMon{\etaWO{\K}}%
                  {F(\Alph_{2})\x \cdots \x F(\Alph_{k})}}
\newcommand{\Kmog}{\SerSAnMon{{\K}_{\mathsf{m}}}{G}}
\newcommand{\Pwog}{\SerSAnMon{\etaWO{\P}}{G}}
\newcommand{\Qwog}{\SerSAnMon{\etaWO{\Q}}{G}}
\newcommand{\QwoZ}{\SerSAnMon{\etaWO{\Q}}{\Z}}
\newcommand{\Qwofa}{\SerSAnMon{\etaWO{\Q}}{F(\Alph)}}
%
\newcommand{\KD}[1]{\SerSAnMon{\K}{#1}}
% Transformation d'Harju Karhumaki 001103
\newcommand{\HKx}[1]{{#1}^{\mathsf{(x)}}}
%%%%%%%%\section{polynomes}
%   Semi-anneaux de polynomes
%
\newcommand{\PolSAnMon}[2]%
    {{#1 \langle  #2 \rangle }}
\newcommand{\PolMon}[1]%
    {{\!\langle  #1 \rangle }}
\newcommand{\SP}[1]{\PolMon{#1}}
%
\newcommand{\KPAe}{\PolSAnMon{\K}{\Ae}}
\newcommand{\KPA}{\KPAe}% compatibility
\newcommand{\KPBe}{\PolSAnMon{\K}{\Be}}
\newcommand{\KPM}{\PolSAnMon{\K}{M}}
\newcommand{\KPN}{\PolSAnMon{\K}{N}}
\newcommand{\KcPN}{\PolSAnMon{\Kcent}{N}}
\newcommand{\KPMN}{\PolSAnMon{\K}{M\x N}}
\newcommand{\KcPMN}{\PolSAnMon{\Kcent}{M\x N}}
\newcommand{\KPNeM}{\PolSAnMon{\left[\KPN\right]}{M}}
\newcommand{\KPMeN}{\PolSAnMon{\left[\KPM\right]}{N}}
\newcommand{\ZPA}{\PolSAnMon{\Z}{\Ae }}
\newcommand{\NPae}{\PolSAnMon{\N}{a^{*}}}
\newcommand{\NPxe}{\PolSAnMon{\N}{x^{*}}}
%
\newcommand{\KPD}[1]{\PolSAnMon{\K}{#1}}
%%% new version 021009
\newsavebox{\LeftBraket}
\savebox{\LeftBraket}{\scalebox{0.7 1.2}{$<$}}
\newsavebox{\RightBraket}
\savebox{\RightBraket}{\scalebox{0.7 1.2}{$>$}}
\newcommand{\bra}[1]{\hbox{}\usebox{\LeftBraket}%
                           #1\usebox{\RightBraket}\hbox{}}
%
\newcommand{\Hank}[1]{H^{({\textstyle{#1}})}}
\newcommand{\Hks}{\Hank{s}}
%%%%%%%%%%%%%%%%%%\section{parties rationnelles}
%   Familles de parties rationnelles
%
\newcommand{\Fin}{\mathrm{Fin}\,}
\newcommand{\Rec}{\mathrm{Rec}\,}
\newcommand{\rec}{\mathrm{Rec}\,} % pour rendre coh\'erentes toutes les notations
\newcommand{\Rat}{\mathrm{Rat}\,}
\newcommand{\rat}{\mathrm{Rat}\,} % pour rendre coh\'erentes toutes les notations
\newcommand{\Rna}{\mathrm{Rna}\,}
\newcommand{\DRat}{\mathrm{DRat}\,}
\newcommand{\DpRat}{\mathrm{D'Rat}\,}
\newcommand{\PRat}{\mathrm{PRat}\,}
\newcommand{\URat}{\mathrm{URat}\,}
\newcommand{\SYn}{\mathrm{Syn}\,}
% \newcommand{\bldRat}{\mathrm{bld-}\Rat}
\newcommand{\bldRat}{\Rat_{\!\!\mathsf{bld}}\,}
%
\newcommand{\Find}{{\Fin _2}}
\newcommand{\Recd}{{\Rec _2}}
\newcommand{\Ratd}{{\Rat _2}}
\newcommand{\bldRatd}{{{\rm bld-Rat}\, _2}}
\newcommand{\DRatd}{{\DRat _2}}
\newcommand{\DpRatd}{{\DpRat _2}}
\newcommand{\Recn}{{\Rec _n}}
\newcommand{\Ratn}{{\Rat _n}}
\newcommand{\DRatn}{{\DRat _n}}
\newcommand{\DpRatn}{{\DpRat _n}}
%
\newcommand{\recc}{{\mathrm{Rec}_2}}   %%%
\newcommand{\rr}{{\mathrm{Rat}_2}}     % sacrifices \`a
\newcommand{\drr}{{\mathrm{DRat}_2}}   % la compatibilit\'e
\newcommand{\drrr}{{\mathrm{D'Rat}_2}} %%%
%
\newcommand{\NRat}{\N \Rat}
\newcommand{\KRat}{\K \Rat}
\newcommand{\BRat}{\B \Rat}
\newcommand{\KRec}{\K \Rec}
\newcommand{\LRec}{\Lb \Rec}
%
\newcommand{\recA}{{{\Rec \Ae}}}
\newcommand{\recB}{{{\Rec \Be}}}
\newcommand{\recC}{{{\Rec \Ce}}}
\newcommand{\ratA}{{{\Rat \Ae}}}
\newcommand{\ratB}{{{\Rat \Be}}}
\newcommand{\ratC}{{{\Rat \Ce}}}
\newcommand{\RecA}{\Rec \Ae}
\newcommand{\RecB}{{{\Rec \Be}}}
\newcommand{\RecC}{{{\Rec \Ce}}}
\newcommand{\RatA}{{{\Rat \Ae}}}
\newcommand{\RatB}{{{\Rat \Be}}}
\newcommand{\RatC}{{{\Rat \Ce}}}
\newcommand{\NRata}{{{\N \Rat \Ae}}}
\newcommand{\PRatA}{{{\PRat \Ae}}}
%\newcommand{\nrata}{{{\N}{\rm Rat}\,\Ae}}
\newcommand{\NRatb}{{{\N \Rat \Be}}}
\newcommand{\Ratbqq}{{(\Rat \Be)^{Q \x Q}}}
\newcommand{\Ratcrr}{{(\Rat \Ce)^{R \x R}}}
\newcommand{\NRatuk}{{{\N \Rat (A_1^* \x \cdots \x A_k^*)}}}
\newcommand{\NRatdk}{{{\N \Rat (A_2^* \x \cdots \x A_k^*)}}}
\newcommand{\RatABe}{{{\Rat \ABe}}}
\newcommand{\ratab}{{{\Rat \ABe}}}
\newcommand{\RecABe}{{{\Rec \ABe}}}
\newcommand{\recab}{{{\Rec \ABe}}}
\newcommand{\dratab}{{{\DRat \ABe}}}
\newcommand{\recac}{{{\Rec (\Ae \x \Ce)}}}
\newcommand{\ratac}{{{\Rat (\Ae \x \Ce)}}}
\newcommand{\dratac}{{{\DRat (\Ae \x \Ce)}}}
%
\newcommand{\utheta}{{U_{\theta }}}
% \newcommand{\umu}{{U_{\mu }}}
\newcommand{\uthetab}{{\OL{U_{\theta }}}}
\newcommand{\umub}{{\OL{U_{\mu }}}}
\newcommand{\vtheta}{{V_{\theta }}}
\newcommand{\vmu}{{V_{\mu }}}
\newcommand{\vthetab}{{\OL{V_{\theta }}}}
\newcommand{\vmub}{{\OL{V_{\mu }}}}
%
%%%%%% \section{repr\'esentation}
% representations
%
\newcommand{\lmn}{{(\lambda , \mu , \nu )}}
\newcommand{\lmnp }{{(\lambda ', \mu ', \nu ')}}
\newcommand{\lmnv}[1]{{(\lambda _{#1}, \mu _{#1}, \nu _{#1})}}
\newcommand{\lmnpv}[1]{{(\lambda' _{#1}, \mu' _{#1}, \nu' _{#1})}}
\newcommand{\lmnu}{{(\lambda _1, \mu _1, \nu _1)}}
\newcommand{\lmnd}{{(\lambda _2, \mu _2, \nu _2)}}
\newcommand{\lmmn}{{\lambda \cdot  m\mu \cdot  \nu }}
\newcommand{\lnmn}{{(\lambda \cdot  n\mu \cdot  \nu )}}
\newcommand{\lfmn}{\lambda \cdot  f\mu \cdot  \nu } % mod. 000601
\newcommand{\lgmn}{{(\lambda \cdot  g\mu \cdot  \nu )}}
\newcommand{\lwmn}{\lambda \cdot  w\mu \cdot  \nu } % mod. 000601
\newcommand{\lumn}{{(\lambda \cdot  u\mu \cdot  \nu )}}
%
\newcommand{\lmnpd}{{({\lambda'} _2, {\mu'} _2, {\nu'} _2)}}
\newcommand{\ekxd}{{(\eta _2,\kappa _2,\xi _2)}}
\newcommand{\ekxpd}{{({\eta'} _2,{\kappa'} _2,{\xi'} _2)}}
\newcommand{\cppd}{{(\chi _2,\pi _2,\psi _2)}}
\newcommand{\cpppd}{{({\chi'} _2,{\pi'} _2,{\psi'} _2)}}
%
\newcommand{\ekz}{{(\eta ,\kappa ,\zeta )}}
\newcommand{\epkpzp}{{(\eta ' ,\kappa ' ,\zeta ' )}}
\newcommand{\ekxv}[1]{{(\eta _{#1},\kappa _{#1},\xi _{#1})}}
\newcommand{\efkz}{{(\eta \cdot f\kappa \cdot \zeta )}}
\newcommand{\lkz}{{(\lambda ,\kappa ,\zeta )}}
\newcommand{\ekx}{{(\eta ,\kappa ,\xi )}}
\newcommand{\ekc}{{(\eta ,\kappa , \chi )}}
\newcommand{\ekxp}{{(\eta' ,\kappa' ,\xi' )}}
\newcommand{\ekxu}{{(\eta _1,\kappa _1,\xi _1)}}
\newcommand{\zso}{{(\zeta ,\sigma ,\omega )}}
\newcommand{\zpo}{{(\zeta , \pi ,\omega )}}
\newcommand{\zsop}{{(\zeta' ,\sigma' ,\omega' )}}
\newcommand{\zsou}{{(\zeta _{1} ,\sigma _{1} ,\omega _{1} )}}
\newcommand{\esx}{{(\eta ,\sigma ,\xi )}}
\newcommand{\esxp}{{(\eta' ,\sigma' ,\xi' )}}
%
\newcommand{\cpp}{{(\chi ,\pi ,\psi )}}
\newcommand{\cppu}{{(\chi _1,\pi _1,\psi _1)}}
\newcommand{\cfpp}{{(\chi \cdot  f\pi \cdot  \psi )}}
%
% representation du (co-)revetement de schutz
\newcommand{\jscol}[1]{| #1 |}
\newcommand{\jsrow}[1]{\underline{\overline{#1}}}
% ???
\newcommand{\jsbin}[2]{{\mathrm{C}_{#1}^{#2}}}
\newcommand{\TS}{\theta\xmd\sigma}
\newcommand{\TSC}{\widehat{\theta\xmd\sigma}}
\newcommand{\RED}{{\mapsto }}
\newcommand{\REDS}{{\stackrel{\star}{\mapsto}}}
\newcommand{\doubleslash}{{/ \! \! \! /}}
% pour matrices prefixes
%   param\'etrisation 010129
\newcommand{\jspbul}{\, \bullet}% compatibilit\'e
% \newcommand{\mpbul}{m_{p \jsSumLigMat }}
% \newcommand{\Mpbul}{M_{p \jsSumLigMat }}
\newcommand{\SommLign}[2]{#1_{#2\, \bullet}}
\newcommand{\mpbul}{\SommLign{m}{p}}
\newcommand{\Mpbul}{\SommLign{M}{p}}
%
% Trace d'une matrice 000607
\newcommand{\Trac}[1]{\mathsf{Tr}(#1)}
%
%%%%%% \section{mono\"\i de libre}
%  monoides libres, monoides, elements neutres de monoides
%  070408 param\'etrisation de l'alphabet
% \renewcommand{\Alph}{A}
% \newcommand{\Blph}{B}
% \newcommand{\Clph}{C}
% \newcommand{\Dlph}{D}
%  990502 param\'etrisation de l'\'etoile
\newcommand{\jsStar}[1]{{{#1}^{*}}}
\newcommand{\Ae}{\jsStar{A}}
\newcommand{\Be}{\jsStar{B}}
\newcommand{\Ce}{\jsStar{C}}
\newcommand{\De}{\jsStar{D}}
\newcommand{\Xe}{\jsStar{X}}
\newcommand{\Ye}{\jsStar{Y}}
\newcommand{\Ze}{\jsStar{Z}}
\newcommand{\jsPlus}[1]{{{#1}^{+}}}
\newcommand{\Ap}{\jsPlus{A}}
\newcommand{\Bp}{\jsPlus{B}}
\newcommand{\Cp}{\jsPlus{C}}
\newcommand{\Dp}{\jsPlus{D}}
\newcommand{\Xp}{\jsPlus{X}}
\newcommand{\Yp}{\jsPlus{Y}}
\newcommand{\Zp}{\jsPlus{Z}}
\newcommand{\azu}{{\{0, 1 \}}}
\newcommand{\azue}{\jsStar{\azu}}
\newcommand{\alphab}{{\{ a, b \}}}
\newcommand{\alphabe}{\jsStar{\alphab}}
\newcommand{\AtA}{{\Alph \x \Alph}}
\newcommand{\AtB}{{\Alph \x \Blph}}
\newcommand{\AtC}{{\Alph \x \Clph}}
\newcommand{\BtC}{{\Blph \x \Clph}}
\newcommand{\AtAe}{\jsStar{(\AtA )}} % erreur corrig\'ee 990916
\newcommand{\AtBe}{\jsStar{(\AtB )}} % idem
\newcommand{\ABe}{{\Ae \x \Be }}
\newcommand{\AAe}{{\Ae \x \Ae }}
\newcommand{\BeBe}{{\Be \x \Be }}
\newcommand{\AuAne}{\Alph_{1}^* \x \Alph_{2}^* \x \cdots \x \Alph_{n}^*}
\newcommand{\AuAke}{\Alph_{1}^* \x \Alph_{2}^* \x \cdots \x \Alph_{k}^*}
\newcommand{\AdAke}{\Alph_{2}^* \x \cdots \x \Alph_{k}^*}
\newcommand{\AedBed}{{\Ae \dol \x \Be \dol}}
\newcommand{\Ace}{{\Ae \x \Ce}}
%%%990421 parametrisation de V(), verbum de
\newcommand{\jsVer}[1]{{\mathrm{V}(#1)}}
\newcommand{\va}{\jsVer{\Ae}}
\newcommand{\vp}{\jsVer{P}}
\newcommand{\vs}{\jsVer{S}}
\newcommand{\vx}{\jsVer{X}}
% alphabets avec dollar pour les relations deterministes
%%%990421 parametrisation
% \newcommand{\dol}{{\small \mbox{$\$ $}}}
% \newcommand{\Adol}{{A_{\dol }}}
\newcommand{\Ad}{\Adol } %compatibilit\'e
% \newcommand{\Bdol}{{B_{\dol }}}
\newcommand{\Bd}{\Bdol } %compatibilit\'e
\newcommand{\AdAde}{{\Adol^* \x \Adol^*}}
\newcommand{\AdBde}{{\Adol ^* \x \Bdol ^*}}
\newcommand{\AdBds}{\AdBde } %compatibilit\'e
% \newcommand{\dol}{{{\scriptstyle \$}}}
%%%%% 990502 rapatriement alphabet morse
\newcommand{\morpoint}{\mbox{\boldmath $\cdot $}}
\newcommand{\mortrait}{\mbox{\hspace{1pt}{\textbf{--}}\hspace{1pt}}}
%%%%% 001114 valeur absolue de diff\'erence de longueurs
\newcommand{\Abso}[1]{\bigl | #1\bigr |}
%%%%%% \section{mon. commutatif libre}
%  monoides commutatif libres
%
\newcommand{\jsStarCom}{\pmb{\oplus}}
\newcommand{\jsCom}[1]{{{#1}^{\jsStarCom}}}
\newcommand{\jsGrCom}[1]{{{#1}^{\circledcirc }}}
\newcommand{\Amc }{\jsCom{\Alph}}
\newcommand{\Bmc }{\jsCom{\Blph}}
\newcommand{\Cmc }{\jsCom{\Clph}}
\newcommand{\Pmc }{\jsCom{P}}
\newcommand{\Nbk }{{\N^{k}}}
% 990502 rapatriement entiers positifs
\newcommand{\Npos}{\N_{*}}
%
% produit de monoides (relations synchronis\'ees)
\newcommand{\dff}{{(\Ae \x \unBe ) \cup (\unAe \x \Be )}}
\newcommand{\dflk}{{(\Alph^{\jsleq k} \x \unBe ) \cup
    (\unAe \x \Blph^{\jsleq k})}}
\newcommand{\dfk}{{(\Alph^{k} \x \unBe ) \cup (\unAe \x \Blph^{k})}}
\newcommand{\Dfk}{{{\mathrm{Diff}_{k}}\,}}
\newcommand{\Dfi}{{{\mathrm{Diff}_{i}}}}
\newcommand{\Dfrat}{{{\mathrm{Diff}_{\mathsf{rat}}}\,}}
\newcommand{\Dfiek}{{{\mathrm{Diff}_{\jsleq k}}}}
\newcommand{\Synm}[1]{{\WT{#1}}}
\newcommand{\Syn}{\mathrm{Syn}}
\newcommand{\Synd}{\mathrm{Syn}_{2}}
\newcommand{\syns}{\Synd}% pour compatibilit\'e
% \newcommand{\syns}{\mbox{$\mbox{{\rm Synch}}_2$}}
\newcommand{\jsCont}[2]{{\mathrm{Cont}_{#1}(#2)}}
\newcommand{\ContR}[1]{\jsCont{R}{#1}}
% \newcommand{\Synn}{{{\mathrm{Syn}_{n}}}}
% \newcommand{\Synu}{{{\mathrm{Syn}_{1}}}}
% \newcommand{\Synnmu}{{{\mathrm{Syn}_{n-1}}}}
\newcommand{\abtb}{\mbox{${\cal A} \bowtie {\cal B}$}}
\newcommand{\abtbu}{\mbox{$({\cal A} \bowtie {\cal B})_1$}}
\newcommand{\abtbd}{\mbox{$({\cal A} \bowtie {\cal B})_2$}}
\newcommand{\adbtb}{\mbox{${\cal A} \db {\cal B}$}}
%
%%%%%% \section{groupe, groupe libre}
%%% 000226 index
\newcommand{\IndGro}[2]{{\pmb{[} #1 \pmb{:}  #2 \,\pmb{]}}}
%%% 001106 commutateur
\newcommand{\Comu}[2]{{\pmb{[} #1 \pmb{,}  #2 \,\pmb{]}}}
%
%%%990421 parametrisation de F(), groupe libre
\newcommand{\jsGL}[1]{{\mathrm{F}(#1)}}
\newcommand{\fga}{\jsGL{\Alph}}
\newcommand{\fgb}{\jsGL{\Blph}}
%%%010103 parametrisation du groupe libre par exposant
% \newcommand{\GLExp}[1]{#1^{\circledast}}
% \newcommand{\GLExp}[1]{#1^{\circ \hspace{-.9ex} \ast}}
\newcommand{\GLExp}[1]{\jsGL{#1}}
\newcommand{\Afg}{\GLExp{\Alph}}
\newcommand{\Bfg}{\GLExp{\Blph}}
% alphabets pour le groupe libre
% 990609 parametrisation jsTil
\newcommand{\jsTil}[1]{\widetilde{#1}}
% \newcommand{\Atil}{\jsTil{A}} dans js_symboles, mais pas param\'etr\'e
\newcommand{\Atileto}{\jsTil{\Alph}^{*}}
\newcommand{\Bte}{\jsTil{\Blph}^{*}}
\newcommand{\unAte}{1_{\Atileto}}
\newcommand{\unFA}{1_{\fga}}
\newcommand{\unFB}{1_{\fgb}}
\newcommand{\unAfg}{1_{\Afg}}
\newcommand{\unBfg}{1_{\Bfg}}
%
\newcommand{\deltau}{\underline{\delta}}
\newcommand{\dyckA}{{D_{\! \! A}^{\, *}}}
\newcommand{\dyckAp}{{D_{\! A}}}
\newcommand{\shamA}{{P_{\! \! A}^{\, *}}}
\newcommand{\shamAp}{{P_{\! A}}}
% symboles pour les simplifications
\newcommand{\Upie}{{U_{\Pi}^{\, *}}}
\newcommand{\Upi}{U_{\ShiftInd{\Pi}}}
\newcommand{\Tpi}{T_{\ShiftInd{\Pi}}}
\newcommand{\Spi}{S_{\ShiftInd{\Pi}}}
% \newcommand{\thetapi}{{\theta _{\Pi}}}
\newcommand{\thetapi}{\theta_{\ShiftInd{\Pi}}}
\newcommand{\etapi}{\eta_{\ShiftInd{\Pi}}}
\newcommand{\pipi}{\pi_{\ShiftInd{\Pi}}}
\newcommand{\iotapi}{\iota_{\ShiftInd{\Pi}}}
\newcommand{\alphapi}{\alpha_{\ShiftInd{\Pi}}}
\newcommand{\iotaK}{\iota_{\ShiftInd{K}}}
\newcommand{\iotaL}{\iota_{\ShiftInd{L}}}
\newcommand{\iotaR}{\iota_{\ShiftInd{R}}}
\newcommand{\iotaT}{\iota_{\ShiftInd{T}}}
\newcommand{\chiK}{\chi_{\ShiftInd{K}}}
%
\newcommand{\dyckrA}{{{D_{\! \! A}'}^{\, *}}} % compat article flavio
%%%%%% \section{app. mon. lib.}
% applications entre monoides libres
\newcommand{\AefAe}{{\Ae \to \Ae}}
\newcommand{\AefBe}{{\Ae \to \Be}}
\newcommand{\AefCe}{{\Ae \to \Ce}}
\newcommand{\BefCe}{{\Be \to \Ce}}
\newcommand{\CefBe}{{\Ce \to \Be}}
\newcommand{\XefYe}{{X^* \to Y^*}}
\newcommand{\ZefAe}{{Z^* \to \Ae}}
\newcommand{\ZefBe}{{Z^* \to \Be}}
\newcommand{\alAB}{{\alpha \colon \Ae \to \Be}}
\newcommand{\betBC}{{\beta \colon \Be \to \Ce}}
\newcommand{\gamAC}{{\gamma \colon \Ae \to \Ce}}
\newcommand{\phiZA}{{\varphi \colon Z^* \to \Ae}}
\newcommand{\psiZB}{{\psi \colon Z^* \to \Be}}
\newcommand{\phiza}{\phiZA} % compatibilit\'e
\newcommand{\psizb}{\psiZB} % compatibilit\'e
% produit avec un element neutre
\newcommand{\AunBe}{{(A \x \{ 1_{\Be} \})}}
\newcommand{\Aeub}{{\Ae \x \{ 1_{\Be} \}}}
\newcommand{\unAeB}{{(\{ 1_{\Ae} \}\x B)}}
\newcommand{\uaBe}{{\{ 1_{\Ae} \}\x \Be}}
\newcommand{\ABgen}{{(A \x \{ 1_{\Be} \})%
                        \cup (\{ 1_{\Ae} \}\x B)}}
\newcommand{\unAe}{{1_{\Ae}}}
\newcommand{\unBe}{{1_{\Be}}}
\newcommand{\unCe}{{1_{\Ce}}}
\newcommand{\unae}{{1_{\Ae}}}
\newcommand{\unbe}{{1_{\Be}}}
\newcommand{\unxe}{{1_{x^*}}}
\newcommand{\uAe}{\unAe} % compatibilit\'e
\newcommand{\uBe}{\unBe} % compatibilit\'e
\newcommand{\Aub}{\AunBe} % compatibilit\'e
\newcommand{\uaB}{\unAeB}
%
\newcommand{\unBde}{{1_{B_{\$}^*}}}
\newcommand{\unAde}{{1_{A_{\$}^*}}}
\newcommand{\AdunBde}{{A_{ \$} \x \{ 1_{B_{\$}^*} \}}}
\newcommand{\unAdBd}{{\{ 1_{A_{\$}^*}}\} \x B_{ \$} }
\newcommand{\uBds}{\unBde}     % compatibilit\'e
\newcommand{\uAds}{\unAde}     % compatibilit\'e papiers
\newcommand{\AduBds}{\AdunBde} % compatibilit\'e Maryse
\newcommand{\uAdsBd}{\unAdBd}  % compatibilit\'e
%%%%%% \section{monoides g\'en\'eraux}
%  monoides g\'en\'eraux, elements neutres de monoides
%
% \newcommand{\unM}{{1_{M}}}
\newcommand{\unM}{{1_{\!M}}}
\newcommand{\unN}{{1_{N}}}
\newcommand{\unG}{{1_{G}}}
\newcommand{\unR}{1_{R}}
\newcommand{\zeU}{{0_{U}}}
\newcommand{\zeV}{{0_{V}}}
\newcommand{\zeW}{{0_{W}}}
\newcommand{\zeM}{{0_{M}}}
%
%%% sous-mono\"\i de engendr\'e % mod 000210\!\!
\newcommand{\jsSMono}[1]{{\pmb{\langle}  #1  \,\pmb{\rangle} }}
% \newcommand{\jsSMono}[1]{{\boldsymbol{\langle}  #1  \,\boldsymbol{\rangle} }}
\newcommand{\ssm}[1]{\jsSMono{#1}} % pour compatibilit\'e
%%% produit direct
\newcommand{\MN}{{M \x N}}
\newcommand{\MNp}{{M' \x N'}}
\newcommand{\Mu}{{M \x 1}}
\newcommand{\uN}{{1 \x N}}
\newcommand{\MP}{{M \x P}}
%
%%%%%% \section{parties de monoides}
\newcommand{\RecM}{{{\Rec M}}}
\newcommand{\RecN}{{{\Rec N}}}
%\newcommand{\recC}{{{\Rec \Ce}}}
\newcommand{\RatM}{{{\Rat M}}}
\newcommand{\RatN}{{{\Rat N}}}
%\newcommand{\ratC}{{{\Rat \Ce}}}
%\newcommand{\NRata}{{{\N \Rat \Ae}}}
% congruences syntaxiques, ensembles de contextes, etc.
\newcommand{\alpharel}{{\mathrel{\alpha }}}
\newcommand{\rhoP}{\mathrel{\rhop}}
\newcommand{\synP}{\mathrel{\sigmap}}
\newcommand{\ConP}[1]{\mathsf{C}_{P}( #1)}
\newcommand{\RConP}[1]{\mathsf{RC}_{P}( #1)}
\newcommand{\RConL}[1]{\mathsf{RC}_{L}( #1)}
\newcommand{\Synt}[1]{{M}_{\ShiftInd{#1}}}
%
% applications entre monoides g\'en\'eraux
\newcommand{\MfN}{{M \to N}}
\newcommand{\MfNp}{{M \to N'}}
%
\newcommand{\alMN}{{\alpha \colon M \to N}}
%\newcommand{\betBC}{{\beta \colon \Be \to \Ce}}
%\newcommand{\gamAC}{{\gamma \colon \Ae \to \Ce}}
%
% pr\'esentation de monoides
\newcommand{\jspre}[2]{%
   {\mbox{$\langle \thinspace #1 \thinspace ;
   \thinspace #2 \thinspace \rangle $}}}
%%%%%% \section{operateurs}
% op\'erateurs et autres symboles compos\'es (970919)
\newcommand{\compos}{\ccdot }
% \newcommand{\xmd}{\,} transf\'er\'e dans js_symboles, avec les espaces
\newcommand{\matmul}{\mathbin{\cdot}}
\newcommand{\minint}{\mathbin{\overset{\cdot}{\smash{-}}}}
% \newcommand{\minint}{\mathbin{\dot{-}}}[-.15ex]\rule{0pt}{.7ex}
% \newcommand{\minint}{\mathbin{\raisebox{0ex}%
%   {$\stackrel{\cdot }{-}$}}}
\newcommand{\starcom }{\oplus }
\newcommand{\prosyn}{\mathbin{\bowtie}}
% op\'erateurs rationnels (020212)
\newcommand{\plusopr}{\mathbin{\mathjsu{+}}}
\newcommand{\prodopr}{\mathbin{\mathjsu{\cdot}}}
\newcommand{\staropr}{\mathbin{\mathjsu{*}}}
%%%%%%%%%%
%%%%%% \section{reductions}
% relations
\newcommand{\jstrans}{\star}
\newcommand{\FTrans}[1]{\mathrel{\overset{\jstrans}{#1}}}
\newcommand{\FTransP}[1]{\mathrel{\overset{+}{#1}}}
\newcommand{\Cong}[1]{\left[#1\,\right]}
\newcommand{\EquR}{\jsSimMist{R}}
\newcommand{\EquRe}{\mathrel{\stackrel{\jstrans}{\EquR }}}
% r\'eductions (commandes generales)
\newcommand{\jsRedu}{\mathrel{%
   \, \rule{0.12ex}{1ex}\rule[0.44ex]{2.2em}{0.12ex} \,}}
\newcommand{\jsRedd}{\mathrel{%
   \, \rule{0.12ex}{1ex}\rule[0.44ex]{2em}{0.12ex} \,}}
\newcommand{\jsRedt}{\mathrel{%
   \, \rule{0.12ex}{1ex}\rule[0.44ex]{1.6em}{0.12ex} \,}}
\newcommand{\jsDerd}{\mathrel{%
   \, \rule[0.44ex]{2.2em}{0.12ex}\rule{0.12ex}{1ex} \,}}
\newcommand{\jsDert}{\mathrel{%
   \, \rule[0.44ex]{1.6em}{0.12ex}\rule{0.12ex}{1ex} \,}}
\newcommand{\jsRedDerd}{\mathrel{%
   \, \rule{0.12ex}{1ex}\rule[0.44ex]{2.2em}{0.12ex}\rule{0.12ex}{1ex} \,}}
\newcommand{\jsRedDert}{\mathrel{%
   \, \rule{0.12ex}{1ex}\rule[0.44ex]{1em}{0.12ex}\rule{0.12ex}{1ex} \,}}
\newcommand{\jsRedDerq}{\mathrel{% incoherence pour compatibilite
   \, \rule{0.12ex}{1ex}\rule[0.44ex]{1.6em}{0.12ex}\rule{0.12ex}{1ex} \,}}
\newcommand{\jsSimu}[1]{\mathrel{\raisebox{-1.6ex}%
  {$\stackrel{\textstyle \jsRedu }{\scriptstyle #1}$}}}
\newcommand{\jsSimd}[1]{\mathrel{\raisebox{-1.6ex}%
  {$\stackrel{\textstyle \jsRedd }{\scriptstyle #1}$}}}
\newcommand{\jsSimt}[1]{\mathrel{\raisebox{-1.6ex}%
  {$\stackrel{\textstyle \jsRedt }{\scriptstyle #1}$}}}
\newcommand{\jsMisd}[1]{\mathrel{\raisebox{-1.6ex}%
  {$\stackrel{\textstyle \jsDerd }{\scriptstyle #1}$}}}
\newcommand{\jsMist}[1]{\mathrel{\raisebox{-1.6ex}%
  {$\stackrel{\textstyle \jsDert }{\scriptstyle #1}$}}}
\newcommand{\jsSimMisd}[1]{\mathrel{\raisebox{-1.6ex}%
  {$\stackrel{\textstyle \jsRedDerd }{\scriptstyle #1}$}}}
\newcommand{\jsSimMist}[1]{\mathrel{\raisebox{-1.6ex}%
  {$\stackrel{\textstyle \jsRedDert }{\scriptstyle #1}$}}}
\newcommand{\jsSimMisq}[1]{\mathrel{\raisebox{-1.6ex}%
  {$\stackrel{\textstyle \jsRedDerq }{\scriptstyle #1}$}}}
% calcul d'une machine 000209
\newcommand{\CalTurA}{\mathrel{\jsSimd{\Ac}}}
\newcommand{\CalTurAe}{\mathrel{\stackrel{\jstrans}{\CalTurA}}}
% d\'eduction logique
\newcommand{\dedjs}{\mathrel{%
   \, \rule{0.12ex}{1.5ex}\rule[0.69ex]{1em}{0.12ex} \,} \ee }
\newcommand{\dedtxt}{\mathrel{%
   \, \rule{0.12ex}{1.5ex}\rule[0.69ex]{1em}{0.12ex} \,}\msp\msp}
% r\'eductions de dyck
\newcommand{\rdyckA}{\jsSimu{\Delta _{A}}}
\newcommand{\rdyck}{\jsSimd{\Delta }}
\newcommand{\redjs}{\jsRedt }
\newcommand{\rdyckAe}{\mathrel{\stackrel{\jstrans}{\rdyckA }}}
\newcommand{\rdycke}{\mathrel{\stackrel{\jstrans}{\rdyck }}}
\newcommand{\redjse}{\mathrel{\stackrel{\jstrans}{\redjs }}}
% r\'eductions de shamir
\newcommand{\rshamA}{\jsSimu{\Sigma _{A}}}
\newcommand{\rshamAe}{\mathrel{\stackrel{\jstrans}{\rshamA }}}
% simplifications
\newcommand{\simpi}{\jsSimt{\Pi}}
\newcommand{\simpie}{\mathrel{\stackrel{\jstrans}{\simpi }}}
\newcommand{\mispi}{\jsMist{\Pi }}
\newcommand{\equpi}{\jsSimMisq{\Pi }}
\newcommand{\equpie}{\mathrel{\stackrel{\jstrans}{\equpi }}}
% 020805 d\'erivation parall\`ele
\newcommand{\jsRedpar}{\mathrel{%
   \, \rule{0.12ex}{1ex}%
   \rule[0.34ex]{1.6em}{0.10ex}%
   \hspace{-1.6em}%
   \rule[0.54ex]{1.6em}{0.10ex}%
   \,}}
\newcommand{\jsSimpar}[1]{\mathrel{\raisebox{-1.6ex}%
  {$\stackrel{\textstyle \jsRedpar }{\scriptstyle #1}$}}}
\newcommand{\simparpi}{\jsSimpar{\Pi}}
\newcommand{\simparpie}{\mathrel{\stackrel{\jstrans}{\simparpi }}}
\newcommand{\simparpik}[1]{\mathrel{\stackrel{#1}{\simparpi }}}
%
% r\'eductions de Buchi
% modif 981227
\newcommand{\jsRedBucu}{\mathrel{%
   \, \rule{0.12ex}{1.2ex}%
   \smash{\makebox[0pt]{\raisebox{-.75ex}{$\,\,\, \scriptscriptstyle \Bc $}}}%
   \rule[0.54ex]{2.5em}{0.12ex} \,}}
\newcommand{\jsRedBucd}{\mathrel{%
   \, \rule{0.12ex}{1.2ex}%
   \makebox[0pt]{\raisebox{-.75ex}{$\,\,\, \scriptscriptstyle \Bc $}}%
   \rule[0.54ex]{2.2em}{0.12ex} \,}}
\newcommand{\rBucK}[1]{\mathrel{\raisebox{-1.6ex}%
  {$\stackrel{\textstyle \jsRedBucu }{\scriptstyle #1}$}}}
\newcommand{\rBucKe}[1]{\mathrel{\stackrel{\jstrans}{\rBucK{#1}}}}
\newcommand{\rBucKn}[2]{\mathrel{\stackrel{#2}{\rBucK{#1}}}}
\newcommand{\rBuc}{\jsRedBucd }
\newcommand{\rBuce}{\mathrel{\stackrel{\jstrans}{\jsRedBucd }}}
%
\newcommand{\REDSP}[1]{\mbox{ $ \stackrel{\star}
{\stackrel{\textstyle \mapsto}{\scriptstyle #1} }$ }}
%%% identit\'es rationnelle comme r\'eduction 020409
\newcommand{\redIdRD}{\mathrel{\msp \jsSimt{\IdRD}\msp}}
\newcommand{\redIdRI}{\mathrel{\msp \jsSimt{\IdRI}\msp}}
\newcommand{\redIdRDe}{\mathrel{\stackrel{\jstrans}{\msp \jsSimt{\IdRD}\msp}}}
\newcommand{\redIdRIe}{\mathrel{\stackrel{\jstrans}{\msp \jsSimt{\IdRI}\msp}}}
%%% interieur de l'inverse
\newcommand{\jsInvInt}[1]{\breve{#1}}
\newcommand{\sigInt}{\jsInvInt{\sigma}}
%%% presentation ???  981015 mod 030211
\newcommand{\jspres}{\, ; \,}
\newcommand{\ETAPres}[2]{\langle \thinspace #1 \thinspace ;
                       \thinspace #2 \thinspace\rangle}
% op\'erations
\newcommand{\Mel}{\mathbin{\between}}
\newcommand{\shuffle}{\mathbin{\circ \! \! \wr }}
\newcommand{\Infil}{\mathbin{\uparrow }}
\newcommand{\infiltration}{\mathbin{\uparrow }}
\newcommand{\kron}{\mathbin{\circ}}
\newcommand{\tensord}{\mathbin{\otimes}} %%% added 061202
\newcommand{\tensor}{\mathbin{\! \otimes \!}}
\newcommand{\tensorsmall}{\mathbin{{\scriptstyle  \otimes }}}
% \renewcommand{\tensorsmall}%
% {\raisebox{0.2ex}{$ \,{\scriptstyle  \otimes } \, $}} %960728
\newcommand{\hadam}{\mathbin{\odot }}
\newcommand{\hadamsmalld}{\mathbin{{\scriptstyle \odot }}}
\newcommand{\hadamsmall}{\mathbin{{\scriptstyle \! \odot \!}}}
\newcommand{\hadamsmallsmall}{\mathbin{{\scriptscriptstyle \odot }}}
\newcommand{\plusMc}{\mathbin{\raisebox{-1ex}%
  {$\, \stackrel{{\scriptstyle +}}{{\scriptscriptstyle \Mc}}\, $}}}
\newcommand{\timesMc}{\mathbin{\raisebox{-1ex}%
  {$\, \stackrel{{\scriptscriptstyle \bullet}}{{\scriptscriptstyle \Mc}}\, $}}}
%
%%%%%% \section{prod morphismes}
\newcommand{\psiA}{\psi_{\ShiftInd{A}}}
\newcommand{\psiC}{\psi_{\ShiftInd{C}}}
\newcommand{\varphiA}{\varphi_{\ShiftInd{A}}}
\newcommand{\varphiC}{\varphi_{\ShiftInd{C}}}
\newcommand{\varphiCi}{\varphi_{\ShiftInd{C}}^{\scriptscriptstyle{-1}}}
\newcommand{\varphiR}{\varphi_{\ShiftInd{R}}}
\newcommand{\tauR}{\tau_{\ShiftInd{R}}}
\newcommand{\psiCi}{\psi_{\ShiftInd{C}}^{\scriptscriptstyle{-1}}}
\newcommand{\phitpsi}{{\mathop{\varphi \x \psi }}}
\newcommand{\phiikpsi}%
{{\varphi ^{-1}\! \compos        \iotaK \! \compos \! \psi }}
\newcommand{\phiiotpsi}[1]%
{{\varphi ^{-1}\! \compos        \iota _{\ShiftInd{#1}} \! \compos \! \psi }}
\newcommand{\phiintkpsi}[1]%
{{(#1\varphi ^{-1}\! \cap K) \psi }}
\newcommand{\mutenskap}{\, \mu \tensorsmall \kappa }
\newcommand{\lamtenseta}{\, \lambda \tensorsmall \eta }
\newcommand{\nutenszet}{\, \nu \tensorsmall \zeta }
\newcommand{\phisuppsi}{{\mathop{\varphi \lor \psi }}}
%
% \section{ordres}
% \renewcommand{\leq}{\leqslant }
\newcommand{\jsleq}{\leqslant }
\newcommand{\jsgeq}{\geqslant }
\newcommand{\jsless}% 001102
   {\mathrel{\leqslant_{\!\!\!\!\scriptscriptstyle{/}}}}
\newcommand{\jsgrea}% 020120
   {\mathrel{\geqslant_{\!\!\!\!\scriptscriptstyle{\backslash}}}}
%
\newcommand{\jsleqpi}{\jsleq_{\ShiftInd{\Pi}}}
\newcommand{\Psipi}[1]{\Psi_{\ShiftInd{\Pi}}^{{\scriptscriptstyle{(#1)}}}}
\newcommand{\Omegapi}[1]{\Omega_{\ShiftInd{\Pi}}^{{\scriptscriptstyle{(#1)}}}}
%
\newcommand{\lexico}{\preccurlyeq }
\newcommand{\lexiconeq}% 010125
   {\preccurlyeq_{\!\!\!\!\!\scalebox{1.8 1}{\scriptscriptstyle{\pmb{/}}}}}
\newcommand{\lexicost}{\lexiconeq}% compatibilit\'e 010125
\newcommand{\nonlexico}{\not \preccurlyeq  }
\newcommand{\ordnat}{\leqslant }
\newcommand{\nonordnat}{\not \leqslant }
\newcommand{\milit}{\sqsubseteq }
% selection et uniformisation 010125
% modif 070303
% \ifenglish
% \newcommand{\jsmil}{\mathsf{rad}}
% \fi
% \iffrench
% \newcommand{\jsmil}{\mathsf{mil}}
% \fi
% modif 100223
\newcommand{\jsmil}{\mathsf{rad}}
\newcommand{\jslex}{\mathsf{lex}}
\newcommand{\Mili}[1]{#1_{\jsmil}}
\newcommand{\Lexi}[1]{#1_{\xmd \jslex}}
\newcommand{\thetamil}{\Mili{\theta}}
\newcommand{\thetalex}{\Lexi{\theta}}
\newcommand{\Mlex}{\Lexi{M}}
%  transfert de js_symboles 001107
\newcommand{\odiveq}{\mathrel{\unlhd}}
\newcommand{\odiv}{\mathrel{\lhd}}
\newcommand{\jsmid}{\mathrel{\big |}}
% \newcommand{\jsmid}{\mathrel{\mid }}
%
%%%%%% \section{automates}
%   automates (modification 970919)
%%%  mod 990114 \langle pour <
%%%  mod 990119 supprim\'e l'espace \;
%%%  mod 061026 supprim\'e l'appel ˆ
%%%             pour Tranah \lrangle de taille variable,
%%%             adaptŽ au contenu
\newcommand{\jsAutUn}[1]%
   {\mbox{$\left\langle \thinspace #1 \thinspace \right\rangle $}}
\newcommand{\aut}[1]{\jsAutUn{#1}} % pour compatibilit\'e
\newcommand{\auta}{\jsAutUn{Q,A,E,I,T}}
\newcommand{\autaf}{\jsAutUn{Q,A,\delta ,I,T}}
\newcommand{\autadet}{\jsAutUn{\PdQ,A,F,\{I\},U}}
\newcommand{\bauta}{\jsAutUn{R,A,F,J,U}}
\newcommand{\autm}{\jsAutUn{Q,M,E,I,T}}
\newcommand{\bautm}{\jsAutUn{R,M,F,J,U}}
\newcommand{\autad}{\jsAutUn{Q,A,E,i,T}}
\newcommand{\autadf}{\jsAutUn{Q,A,\delta ,i,T}}
\newcommand{\autv}[3]{\jsAutUn{#1 , #2  , #3}}
\newcommand{\autiet}{\jsAutUn{I, E ,T}}
\newcommand{\autjfu}{\jsAutUn{J, F ,U}}
% aut gauche et droit 990519
\newcommand{\jsGSymb}{\rightsquigarrow}
\newcommand{\jsDSymb}{\scalebox{-0.9 0.9}{\jsGSymb}}
\newcommand{\jsAutG}[1]{\overset{\jsGSymb}{#1}}
\newcommand{\jsAutD}[1]{\overset{\jsDSymb}{#1}}
%  001114  transitions
\newcommand{\Tran}[1]{\bigl ( #1\bigr )}
%%% \'etiquette de transducteur: entr\'ee et sortie
% pour le texte mod de la macro dans Vaucanson 010104
\newcommand{\IOLt}[2]{#1\mid #2}
%   2-automates
\newcommand{\autab}{\jsAutUn{Q,A,B,E,I,T}}
% transposition 000118 % 020223
\newcommand{\jsTrsp}[1]{#1^{\mathsf{t}}}
% normalisation 990524 mod 990711
\newcommand{\jsNorm}[1]{{#1_{\mathsf{nor}}}}
% normalisation pour morphisme 000215
\newcommand{\NormMor}[1]{{#1_{\mathsf{n}}}}
% \'emondation 990524
\newcommand{\jsEmon}[1]{{#1_{\mathsf{m}}}}%\acute{e}
% compl\'etion  991212
\newcommand{\AutComp}[1]{{{#1}_{\mathsf{c}}}}
% compl\'ement  020206
\newcommand{\AutCpl}[1]{{#1}^{\mathsf{c}}}
% complexit\'e n \'etats  020521
\newcommand{\StatComp}[1]{\mathsf{Sc}({#1})}
%% determinisation (modification 980417)
% mod 990711 remplacement de \Dc
% mod 991214 sur le modele des \jsEmon, etc.
\newcommand{\jsdet}{\mathsf{det}}
\newcommand{\jscod}{\mathsf{cod}}
\newcommand{\jsDeter}[1]{{{#1}_{\jsdet}}}%
\newcommand{\jsCodet}[1]{{{#1}_{\jscod}}}%
\newcommand{\Acdet}{\jsDeter{\Ac}}%{{\Ac_{\jsdet }}}
\newcommand{\Accod}{\jsCodet{\Ac}}%{{\Ac_{\jscod }}}
\newcommand{\Acu}{{{\Ac_{1}}}}
\newcommand{\Acudet}{\jsDeter{\Acu}}%{{{\Ac_{1}}_{\jsdet }}}
\newcommand{\piaud}{{\pi_{\Acudet}}}
\newcommand{\pibu}{{\pi_{\Bc_{1}}}}
%% bouquets (modification 971016,990907)
% 000215 passage en sans serif
\newcommand{\jsOut}[2]{{{\mathsf{Out}}_{#1}( #2)}}
\newcommand{\jsIn}[2]{{{\mathsf{In}}_{#1}( #2)}}
% \newcommand{\jsOut}[2]{{{\rm Out}_{#1}( #2)}}
% \newcommand{\jsIn}[2]{{{\rm In}_{#1}( #2)}}
%
\newcommand{\outa}[1]{\jsOut{\Ac}{#1}}
\newcommand{\outat}[1]{\jsOut{\jsTrsp{\Ac}}{#1}}
\newcommand{\outb}[1]{\jsOut{\Bc}{#1}}
\newcommand{\outc}[1]{\jsOut{\Cc}{#1}}
\newcommand{\outab}[1]{\jsOut{\Ac \x \Bc}{#1}}
\newcommand{\outba}[1]{\jsOut{\Bc \x \Ac}{#1}}
%
\newcommand{\ina}[1]{\jsIn{\Ac}{#1}}
\newcommand{\inb}[1]{\jsIn{\Bc}{#1}}
\newcommand{\stara}[1]{{{\rm Star}_{\Ac}( #1)}}
\newcommand{\costara}[1]{{{\mathrm{co-Star}}_{\Ac}( #1)}}
%% \section{passe-present-futur} (971030)
% 000215 passage en sans serif
% 020712 mod sur l'indice
\newcommand{\jsPast}[2]{{\mathsf{Past}}_{\ShiftInd{#1}}(#2)}
\newcommand{\jsPres}[2]{{\mathsf{Pres}}_{\ShiftInd{#1}}(#2)}
\newcommand{\jsFut}[2]{{\mathsf{Fut}}_{\ShiftInd{#1}}(#2)}
\newcommand{\jsTrans}[2]{{\mathsf{Trans}}_{\ShiftInd{#1}}(#2)}
%
\newcommand{\pasta}[1]{\jsPast{\Ac}{#1}}
\newcommand{\pastv}[1]{\jsPast{\Vc}{#1}}
\newcommand{\presa}[1]{\jsPres{\Ac}{#1}}
\newcommand{\futa}[1]{\jsFut{\Ac}{#1}}
\newcommand{\futv}[1]{\jsFut{\Vc}{#1}}
\newcommand{\transa}[1]{\jsTrans{\Ac}{#1}}
\newcommand{\futacb}[1]{\jsFut{\Ac_{CB}}{#1}}
%
\newcommand{\pastuk}[1]{\jsPast{\Uc_{K}}{#1}}
\newcommand{\futuk}[1]{\jsFut{\Uc_{K}}{#1}}
%% automate universel (020711)
\newcommand{\ShiftInd}[1]{\raisebox{-0.3ex}{$\scriptstyle{#1}$}}
\newcommand{\SymbWShiftInd}[2]{#1_{\ShiftInd{#2}}}% mod 020722
\newcommand{\RaiseExp}[1]{\raisebox{0.3ex}{$\scriptstyle{\,#1}$}}
%
\newcommand{\Univ}[1]{\Uc_{\ShiftInd{#1}}}
\newcommand{\EFac}[1]{E_{\ShiftInd{#1}}}
\newcommand{\FFac}[1]{F_{\ShiftInd{#1}}}
\newcommand{\IFac}[1]{I_{\ShiftInd{#1}}}
\newcommand{\QFac}[1]{Q_{\ShiftInd{#1}}}
\newcommand{\TFac}[1]{T_{\ShiftInd{#1}}}
\newcommand{\Univrel}[2]{\Uc_{\ShiftInd{#1}}^{{\scriptscriptstyle{(#2)}}}}
\newcommand{\EFacrel}[2]{E_{\ShiftInd{#1}}^{{\scriptscriptstyle{(#2)}}}}
\newcommand{\FFacrel}[2]{F_{\ShiftInd{#1}}^{{\scriptscriptstyle{(#2)}}}}
%
\newcommand{\Uk}{\SymbWShiftInd{\Uc}{K}}
\newcommand{\Ek}{\SymbWShiftInd{E}{K}}
\newcommand{\Fk}{\SymbWShiftInd{F}{K}}
\newcommand{\Ik}{\SymbWShiftInd{I}{K}}
\newcommand{\Qk}{\SymbWShiftInd{Q}{K}}
\newcommand{\Tk}{\SymbWShiftInd{T}{K}}
\newcommand{\Ekg}{\EFacrel{K}{G}}
\newcommand{\Fkg}{\FFacrel{K}{G}}
\newcommand{\Uka}{\Univrel{K}{A}}
\newcommand{\Ukg}{\Univrel{K}{G}}
\newcommand{\Eke}{E_{K}^{\raisebox{0.3ex}{$\scriptstyle{\,*}$}}}
\newcommand{\Ekp}{E_{K}^{\raisebox{0.3ex}{$\scriptstyle{\,+}$}}}
\newcommand{\Fke}{F_{K}^{\raisebox{0.3ex}{$\scriptstyle{\,*}$}}}
\newcommand{\Fkp}{F_{K}^{\raisebox{0.3ex}{$\scriptstyle{\,+}$}}}
%
\newcommand{\Qp}{\SymbWShiftInd{Q}{P}}
\newcommand{\rhop}{\SymbWShiftInd{\rho}{P}}
\newcommand{\sigmap}{\SymbWShiftInd{\sigma}{P}}
%
\newcommand{\Expan}[1]{{#1}_{\ShiftInd{\text{\rmfamily{CB}}}}}
\newcommand{\Acb}{\Expan{\Ac}}
%%%%%% \section{actions}
% action d'un mono\"\i de sur un ensemble (modif 971019)
\newcommand{\ActMor}[1]{\overset{{\scriptscriptstyle \pmb{\lor}}}{#1}}%
% \newcommand{\ActMor}[1]{\check{#1}}%
\newcommand{\act}{\mathbin{\boldsymbol{\cdot}}}
% \newcommand{\act}{\mathbin{\pmb{\cdot}}}
\newcommand{\actseq }{\mathbin{*}}
\newcommand{\jsAct}[1]{\mathbin{\raisebox{-1ex}{$%
  \stackrel{\boldsymbol{\cdot}}%
%   \stackrel{\pmb{\cdot}}%
      {\makebox[0pt][c]{${\scriptscriptstyle \rule{0pt}{0.7ex} \smash[t]{ #1}}$}}$}
          }}
\newcommand{\jsActW}[1]{\mathbin{\raisebox{-1ex}{$%
  \stackrel{\boldsymbol{\cdot}}%
%   \stackrel{\pmb{\cdot}}%
      {\makebox[0.8\width][c]{${\scriptscriptstyle \rule{0pt}{0.7ex} \smash[t]{ #1}}$}}$}
          }}
\newcommand{\actM}{\jsAct{M}}
\newcommand{\actS}{\jsAct{S}}
\newcommand{\actT}{\jsAct{T}}
\newcommand{\actAccod}{\jsAct{\Accod}}
%% fausse action (transducteur d\'eterministe) 990621
\newcommand{\actb}{\mathbin{\raisebox{0.2ex}%
                        {${\scriptscriptstyle \circ} $}}}
\newcommand{\ccdot}{\actb} % pour compatibilit\'e
% action Avance ou Retard  990802
\newcommand{\ADzero}{\pmb{\mathsf{0}}}
\newcommand{\ZeroAAR}{\ADzero} % pour compatibilit\'e
% macros parametrees 991124
\newcommand{\ADbase}[1]{H_{#1}}
\newcommand{\ADbB}{\ADbase{B}}
\newcommand{\ADact}[1]{\omega_{#1}}
\newcommand{\ADaB}{\ADact{B}}
%% automate d'une action
\newcommand{\Ddel}{\SymbWShiftInd{\Dc}{\delta}}
\newcommand{\DFacrel}[2]{\Dc_{\ShiftInd{#1}}^{{\scriptscriptstyle{(#2)}}}}
\newcommand{\Ddelg}{\DFacrel{\delta}{G}}
%% applications indicees (971030)
\newcommand{\psiM}{{\psi _{M}}}
\newcommand{\psiN}{{\psi _{N}}}
\newcommand{\psiAe}{{\psi _{\Ae}}}
%
\newcommand{\pia}{{\pi_{\Ac}}}
\newcommand{\piap}{{\pi_{\Ac'}}}
\newcommand{\piad}{{\pi_{\Acdet}}}
\newcommand{\piacd}{{\pi_{\Accod}}}
\newcommand{\pib}{{\pi_{\Bc}}}
%
\newcommand{\LpA}{{L_p(\Ac)}}
\newcommand{\LqA}{{L_q(\Ac)}}
\newcommand{\LiA}{{L_i(\Ac)}}
%
\newcommand{\dil}{{\delta_{1}^{L}}}
\newcommand{\dpT}{{\delta_{p,T}}} %000521
\newcommand{\dpt}{\dpT} %000521
\newcommand{\dpI}{{\delta_{p,I}}} %000521
%% param\'etrisation - mod pour trans. det. (990620)
%% 100724 new design of \CompAuto, in order
%% to avoid \pmb which behaves strangely.
%% Open the way to variable size version.
\newlength{\vbh}\newlength{\vbd}\newlength{\vbt}%
% \settodepth{\vbd}{\strut}\settoheight{\vbh}{\strut}\setlength{\vbt}{\vbh}%
% \addtolength{\vbt}{\vbd}%
\newcommand{\CompAuto}[1]%
    {%
     \settodepth{\vbd}{\mbox{$\displaystyle{#1\strut}$}}%
     \settoheight{\vbh}{\mbox{$\displaystyle{#1\strut}$}}%
     \setlength{\vbt}{\vbh}\addtolength{\vbt}{\vbd}%
     {}%
     \psline[linewidth=0.8pt]{c-c}(0,-.65\vbd)(0,.9\vbh)%
%      \strut\kern0.7pt%
     \hspace*{0.7pt}%
     {#1}%
     \kern0.8pt%
     \psline[linewidth=0.8pt]{c-c}(0,-.65\vbd)(0,.9\vbh)%
     }%
% \newcommand{\CompAuto}[1]{{\pmb{|}{#1}\pmb{|}}}
%%% 071110 compAuto with small space on the right
\newcommand{\CompAutoRS}[1]{\pmb{|}{#1}\xmd\pmb{|}}
\newcommand{\compaut}[1]{\CompAuto{#1}}  % pour compatibilit\'e
\newcommand{\compA}{\CompAuto{\Ac}}
\newcommand{\compB}{\CompAuto{\Bc}}
\newcommand{\compT}{\CompAuto{\Tc}}
\newcommand{\compautv}[3]{\CompAuto{\jsAutUn{#1 , #2  , #3 }}}
\newcommand{\CompHBal}[1]{{\CompAuto{#1}_{\dol}}}
\newcommand{\compAdol}{\CompHBal{\Ac}}
\newcommand{\compTdol}{\CompHBal{\Tc}}
\newcommand{\DCompAuto}[1]{{|{#1}|}} %????
\newcommand{\compdaut}[1]{\DCompAuto{#1}} % pour compatibilit\'e
\newcommand{\compdA}{\DCompAuto{\Ac}}
%%%%%% \section{McNaugton}
\newcommand{\mBC}[2]{{\mathjsu{E}}^{(#1)}(#2)}% _{\BzCi}
\newcommand{\mMNY}[2]{{\mathjsu{M}}^{(#1)}_{#2}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bornedeuxlignes}[2]%
{\mbox{$
\renewcommand{\arraystretch}{0.5}%
\begin{array}{c}{\scriptstyle #1}\\ {\scriptstyle #2} \end{array}
\renewcommand{\arraystretch}{2}%
       $}}
% \newcommand{\bdl}[2]{\bornedeuxlignes{#1}{#2}}
%% modif 000825
\newcommand{\bdl}[2]{%
\makebox%
% [0pt]
% [\width{%
% \mbox{$
% \scriptstyle #1
% $}
% }]%
% [c]%
{$ \renewcommand{\arraystretch}{0.5}%
\begin{array}{c}{\scriptstyle #1}\\ {\scriptstyle #2} \end{array}%
\renewcommand{\arraystretch}{2} $}}
%
\newcommand{\bdld}[2]{%
   \makebox{$ \renewcommand{\arraystretch}{0.66667}%
   \begin{array}{c}{\scriptstyle #1}\\ {\scriptstyle #2} \end{array}%
   \renewcommand{\arraystretch}{1.5} $}}
%%%%%% \section{chemins}
% d\'eclaration de chemins
\newcommand{\eqcal}{\mathrel{\; : = \; }\ }
% 990521 version fleche extensible, merci marie-pierre
% \newcommand{\path}[1]{\xrightarrow{\ #1 \ }} %100309 pb
\renewcommand{\path}[1]{\xrightarrow{\ #1 \ }} %100309 pb
\newcommand{\pathaut}[2]{\underset{#2}{\path{#1}}}
% \newcommand{\path}[1]{\stackrel{#1}{\longrightarrow}}
% \newcommand{\pathaut}[2]{\raisebox{-1.3ex}{ $ \stackrel{#1}
% {\stackrel{\textstyle \longrightarrow}{\scriptstyle #2} }$ }}
\newcommand{\pathl}[1]{@>{#1}>>}
\newcommand{\pathlaut}[2]{@>{#1}>{#2}>}
%%%%%% \section{expressions}
\newcommand{\RatE}{\mathjsu{RatE}\,}% mod. 020212
\newcommand{\URatE}{\mathjsu{URatE}\,}% mod. 020413
\newcommand{\GRatE}{\mathjsu{GRatE}\,}% mod. 020413
\newcommand{\Ratx}{\RatE}
\newcommand{\URatx}{\URatE}
\newcommand{\GRatx}{\GRatE}
\newcommand{\RatEA}{\mathjsu{RatE}\,\Ae}% mod. 020430,030123
\newcommand{\RatExp}[2]{{#1\,\mathjsu{RatE}\,#2}}
\newcommand{\KRA}{\RatExp{\K}{\Ae}}
\newcommand{\KREM}{\RatExp{\K}{M}}
%   expressions (d\'ebut 000201)
% \newcommand{\TermCst}[1]{{\operatorname{\mathsf{c}}(#1)}}
\newcommand{\GTermCst}[1]{\operatorname{\mathsf{c}}\left(#1\right)}
% mise en sans serif le 000510
\newcommand{\Dpth}[1]{\operatorname{\mathsf{d}}(#1)}
\newcommand{\Depth}[1]{\Dpth{#1}} %compatibility
%% version broken derived terms
%%%%%% \section{expression derivation}
\newcommand{\Kron}[1]{\delta_{#1}}
\newcommand{\PropSet}[1]{#1_{\mathsf{p}}}
\newcommand{\PropSetP}[1]{\left(#1\right)_{\mathsf{p}}}
\newcommand{\properset}[1]{\PropSetP{#1}}
%
\newcommand{\ExpDer}[2][a]%
    {\operatorname{\frac{\partial}{\partial \mbox{$#1$}}}#2}
\newcommand{\ExpDerP}[2][a]%
    {\operatorname{\frac{\partial}{\partial\mbox{$#1$}}}\left(#2\right)}
%
% \newcommand{\ExpDerB}[2][a]% 020429
%    {{\operatorname{\frac{\partial '}{\partial '\mbox{$#1$}}}#2}}
%
\newcommand{\ExpDerr}[2][a]%
    {\operatorname{\frac{\partial_{\mathrm{R}}}{\partial \mbox{$#1$}}}#2}
\newcommand{\ExpDerB}[2][a]%
   {\operatorname{\frac{\partial_\mathsf{b}}{\partial \mbox{$#1$}}}#2}
\newcommand{\ExpDerBP}[2][a]%
   {\operatorname{\frac{\partial_\mathsf{b}}{\partial \mbox{$#1$}}}\left(#2\right)}
%%%%%% {derived terms}
\newcommand{\TerScale}{0.9}
%
\newcommand{\DTer}{\scalebox{\TerScale}{\mathrm{D}}}
\newcommand{\TDTer}{\scalebox{\TerScale}{\mathrm{TD}}}
%
\newcommand{\DerTer}[1]{{\DTer}\left(#1\right)}
\newcommand{\DerTerSub}[1]{{\mathrm{D}}\left(#1\right)}
\newcommand{\TruDerTer}[1]{{\TDTer}\left(#1\right)}
\newcommand{\TruDerTerSub}[1]{{\mathrm{TD}}\left(#1\right)}
%%%%%% {broken derived terms}
\newcommand{\BTer}{\scalebox{\TerScale}{\mathrm{B}}}
\newcommand{\BDTer}{\scalebox{\TerScale}{\mathrm{BD}}}
\newcommand{\TBDTer}{\scalebox{\TerScale}{\mathrm{TBD}}}
%
% \newcommand{\InitDer}[1]{\operatorname{\mathrm{d}}\!\left(#1\right)}
% \newcommand{\InitDerSub}[1]{\operatorname{\mathrm{d}}\left(#1\right)}
\newcommand{\InitDer}[1]{{\BTer}\left(#1\right)}
\newcommand{\InitDerSub}[1]{\mathrm{B}\left(#1\right)}
\newcommand{\DerTerB}[1]{{\BDTer}\left(#1\right)}
\newcommand{\DerTerBSub}[1]{{\mathrm{BD}}\left(#1\right)}
\newcommand{\TruDerTerB}[1]{{\TBDTer}\left(#1\right)}
\newcommand{\TruDerTerBSub}[1]{{\mathrm{TBD}}\left(#1\right)}
%
\newcommand{\DerTerw}[1]{\DerTer[w]{#1}}
%
\newcommand{\NomDer}[1]{{\operatorname{bf{nd}}(#1)}}
%%% complement 000103 pour expression generalis\'ee
\newcommand{\CompExp}[1]{\OL{#1}}% malheureux! 020413
%%%
% \newcommand{\CompExpr}[1]{{\pmb{|}{#1}\pmb{|}}}
\newcommand{\CompExpr}[1]{\CompAuto{#1}}
%
\newcommand{\Kadd}{\oplus}
\newcommand{\Ksum}{\bigoplus}
\newcommand{\LitLength}{\operatorname{\ell}}
\newcommand{\LitL}[1]{\LitLength (#1)}
\newcommand{\VCoef}[3]{{#2}^{\scriptscriptstyle (#1)}_{#3}}
\newcommand{\kCoef}[2][a]{{k}^{{\scriptscriptstyle (#1)}}_{#2}}
\newcommand{\kfCoef}[2][f]{{k}^{{\scriptscriptstyle (#1)}}_{#2}}
\newcommand{\lCoef}[2][a]{{l}^{{\scriptscriptstyle (#1)}}_{#2}}
\newcommand{\zCoef}[2][a]{{z}^{{\scriptscriptstyle (#1)}}_{#2}}
\newcommand{\ICoef}[2][a]{{I}^{{\scriptscriptstyle (#1)}}_{#2}}
\newcommand{\JCoef}[2][a]{{J}^{{\scriptscriptstyle (#1)}}_{#2}}
\newcommand{\HCoef}[2][a]{{H}^{{\scriptscriptstyle (#1)}}_{#2}}
\newcommand{\SCoef}[2][a]{{S}^{{\scriptscriptstyle (#1)}}_{#2}}
\newcommand{\RCoef}[2][a]{{R}^{{\scriptscriptstyle (#1)}}_{#2}}
\newcommand{\QCoef}[2][a]{{Q}^{{\scriptscriptstyle (#1)}}_{#2}}
%%%%%% \section{produit libre}
%  Produits libres
% mod et param\'etrisation 000830
\newcommand{\ETAmun}[1]{{#1}_{\bullet}}
\newcommand{\Mmun}{\ETAmun{M}}
\newcommand{\Nmun}{\ETAmun{N}}
% \newcommand{\Mmun}{{ M^\bullet }}
% \newcommand{\Nmun}{{ N^\bullet }}
\newcommand{\MlN}{{ M \! * \! N }}
\newcommand{\unMlN}{1_{\MlN}}
\newcommand{\MlNi}{{ \scriptstyle{M \! * \! N} }}
\newcommand{\philpsi}{{ \varphi \! * \! \psi }}
\newcommand{\MlNmun}{{ (M \! * \! N)^\bullet }}
\newcommand{\MAT}{{ {\rm M} (A,\theta ) }}
\newcommand{\MI}{{\rm MI}}
\newcommand{\MF}{{\rm MF}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\endinput

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

